Universality of max-margin classifiers

Maximum margin binary classification is one of the most fundamental algorithms in machine learning, yet the role of featurization maps and the high-dimensional asymptotics of the misclassification error for non-Gaussian features are still poorly understood. We consider settings in which we observe binary labels $y_i$ and either $d$-dimensional covariates ${\boldsymbol z}_i$ that are mapped to a $p$-dimension space via a randomized featurization map ${\boldsymbol \phi}:\mathbb{R}^d \to\mathbb{R}^p$, or $p$-dimensional features of non-Gaussian independent entries. In this context, we study two fundamental questions: $(i)$ At what overparametrization ratio $p/n$ do the data become linearly separable? $(ii)$ What is the generalization error of the max-margin classifier? Working in the high-dimensional regime in which the number of features $p$, the number of samples $n$ and the input dimension $d$ (in the nonlinear featurization setting) diverge, with ratios of order one, we prove a universality result establishing that the asymptotic behavior is completely determined by the expected covariance of feature vectors and by the covariance between features and labels. In particular, the overparametrization threshold and generalization error can be computed within a simpler Gaussian model. The main technical challenge lies in the fact that max-margin is not the maximizer (or minimizer) of an empirical average, but the maximizer of a minimum over the samples. We address this by representing the classifier as an average over support vectors. Crucially, we find that in high dimensions, the support vector count is proportional to the number of samples, which ultimately yields universality.

==> 4_sep_loss_old.tex <==


\newpage
\section{Universality of the surrogate loss}

%\notate{To be removed}
%Let us define for $|s|\le s_0$, $L>0$, $l\in\{1,2,3\}$, define the max-margin
%\begin{equation}
%\widehat\kappa_{l,s,L,R}^\bX := \max_{\theta \in S_l(s,L,R)}  \min_{i \in[n]} y_i(\bx_i) \btheta^\sT\bx_i.
%\end{equation}
%Additionally, for $\kappa >0$
%on the event 
%\begin{equation}
%\cG_{l,s,L,R} := \{ \exists \btheta : S_l(s,L,R) \neq \emptyset \},
%\end{equation}
%define
%\begin{equation} 
%\widehat H_{l,s,L,R}^\bX(\kappa) := \min_{\{\btheta : y_i(\bx_i)\bx_i^\sT\btheta \ge \kappa\}} \norm{\btheta}_2^2 + s C_l(\btheta).
%\end{equation}
%
%
%
%\begin{equation}
% s_0(\kappa) =  \frac12\left( \frac{\kappa}{\sfK\oslambda}  \wedge \frac1\oslambda \wedge \oslambda\right),
%\end{equation}
%\notate{need to ensure that $s_0 \le \norm{\bX}_\op / \sqrt{n}$  w.h.p.}
The goal of this section is to prove the universality of the minimum of the surrogate loss for the max-margin problem over appropriate sets.
Before stating the main result of the section, let us define the perturbation functions
\begin{equation}
  \pi_1(\btheta) := \btheta^\sT\bSigma \btheta^\star,
  \quad 
  \pi_2(\btheta) := \norm{\btheta}_\Sigma^2,
  \quad 
  \pi_3(\btheta) := \norm{\btheta}_4^4
\end{equation}
and the associated constraint sets
\begin{equation}
 \cS_l(s,b_1) := \{\btheta : \norm{\btheta}_2^2 + s\pi_l(\btheta)\le b_1, \norm{\btheta}_2^2 \le b_2(l,b_1)\}
\end{equation}
where
\begin{equation}
 b_2(1, b_1) = \frac{s_0 + \sqrt{s_0^2\oslambda^2 \norm{\btheta^\star}_2^2 + 4 b_1}}{2} ,
 \quad
 b_2(2,b_1 ) = \frac{b_1  + 1}{1 - s_0 \oslambda},
 \quad 
 b_2(3,b_1) \notate{Fill}.
\end{equation}


Define the associated surrogate minimization problems
\begin{equation} 
\widehat F_{l}^\sur(\bD;\kappa, s ,b_1) := \min_{\btheta \in \cS_l(s,b_1,b_2)} 
L^{\sur}(\bD, \btheta ; \kappa )
\quad
L^\sur(\bD, \btheta ; \kappa) :=\frac1n \sum_{i=1}^n \left(\kappa - y_i(\bd_i)\btheta^\sT\bx_i \right)_+^2
\end{equation}
for $l\in\{1,2\}$, $|s| \le s_0$  and $b_1 > 0$.


We will prove the following claim.
\begin{theorem}
\label{thm:univ_fixed_kappa}
Assume there exists universal constants $C_i >0$ such that
 $\oslambda := \norm{\bSigma}_\op  \le C_0$, $\norm{\btheta^\star}_2 \le C_1$, $\norm{\Sigma \btheta^\star}_\infty \le C_2 n^{-\delta}$ for some $\delta>0$.
Fix $|s| \le 1, b_1 > 0,\kappa >0$. 
Let $\cS_l := \cS_l(s,b_1,b_2)$
and $b_2= b_2(l, b_1)$ as above
for $l\in\{1,2,3\}$.
We have for all bounded Lipschitz functions
$\varphi$,
\begin{equation}
\lim_{n\to\infty}
\left|\E\left[\varphi\left(\widehat F_{l}(\bX;\kappa, s, b_1,b_2)\right) \right]
-
\E\left[\varphi\left(
\widehat F_{l}(\bG;\kappa, s, b_1,b_2)\right) \right]
\right| = 0
\end{equation}
as $n\to\infty$ with $p/n \to \psi$.
\end{theorem}
In this section, we establish this theorem as a corollary of [MS22] by reducing it to their assumptions.
In Section~\ref{}, we show that adding an $\ell^2$ regularizer to the problem changes the minimum by only a small amount. Then, in Section~\ref{}, 
we show that this this regularized, strongly convex problem can be reduced to one where the loss is Lipschitz instead of quadratic, satisfying the assumptions of [MS22].
We then check that the minimizer, with high probability, will have a small $\ell^\infty$ norm allowing us to conclude that the well-spreadedness assumption of [MS22] holds.
Finally, since we are dealing with a setting where the labels $\by$ are functions of the latent variables $\bz$ in the random features model, we augment the features in Section~\ref{} 
to reduce to the setting there the labels are a direct function of the feature vectors.

Throughout the remainder of this section, we suppress the dependence in notation on parameters that are considered fixed in the respective section, whenever it is convenient to do so without confusion.
For example, we write $\widehat F^\sur_l(\bD)$ instead of explicating its dependence on $\kappa,s$ and $b_1$.
%\section{TEMP}
%\notate{CHeck the conditions of the sets $S$ in the surrogate universality lemma}
%
%Let $G(\btheta)$ be a differentiable convex function such that $G(\btheta) \ge C \norm{\btheta}_2^2 $ for some 
%$C>0$. Note that the functions 
%$\btheta \mapsto \norm{\btheta}_2^2 + s C_l(\btheta)$ satisfy this. 
%Indeed, verifying convexity is straightforward using the spectrum condition on $\bSigma$ and the 
%domain of $s$. Meanwhile,
%if $\norm{\btheta}_2^2 + s C_l(\btheta) \le L$, we have for $l=1$
%\begin{equation}
% \norm{\btheta}_2 \le \frac{1 + (1+4L)^{1/2}}{2} =: C_0(L)
%\end{equation}
%and for $l=2$ 
%\begin{equation}
% \norm{\btheta}_2 \le \left(\frac{L}{1-|s| \overline\slambda}\right)^{1/2} \le 
% \left(2 L\right)^{1/2} := C_1(L).
%\end{equation}
%


\subsection{Approximation with a regularized problem}
The first step is to show that we can approximate the minimization problem uniformly with an 
$\ell_2$ regularized problem 
\begin{equation}
\label{eq:reg_problem}
 \widehat F_l^{\rm{reg}}(\bD; \lambda):= \min_{\btheta \in \cS_l} L^\reg(\btheta;\lambda)
 \quad L^\reg(\btheta) := \frac1n \sum_{i=1}^n 
 \left(\kappa - y_i\bd_i^\sT\btheta\right)_+^2 + \frac{\lambda}{2} \norm{\btheta}_2^2.
\end{equation}
The following lemma establishes the validity of this approximation.
\begin{lemma}
Let $\kappa,s,b_1,b_2$ be as in Theorem~\ref{thm:univ_fixed_kappa}.
For $l\in\{1,2,3\}$, we have for all bounded Lipschitz functions $\varphi$ and all $\lambda>0$,
\begin{equation}
\lim_{n\to\infty} \left|\E\left[\varphi\left(\widehat F_l^{\rm{reg}}(\bD; \lambda)\right)\right] 
-
\E\left[\varphi\left(\widehat 
F_l^{\sur}(\bD)\right)\right]
\right| \le  \frac{b_2\norm{\varphi}_\Lip}2  \lambda.
\end{equation}
\end{lemma}
\begin{proof}
Let $\widehat\btheta(\lambda)$ be the minimizer of the problem in~\eqref{eq:reg_problem}.
Note that we have both
\begin{equation}
     L^\reg(\widehat\btheta(\lambda);\lambda)
 \ge L^\reg(\widehat\btheta(\lambda); 0)
 \ge L^\reg(\widehat\btheta(0); 0)\quad \textrm{and}\quad
L^\reg(\widehat \btheta(\lambda); \lambda) \le  
L^\reg(\widehat \btheta(0); \lambda) \le 
L^\reg(\widehat \btheta(0); 0) + \frac\lambda2 b_2.
\end{equation}
since $\widehat\btheta(0) \in \cS_l$ implies $\big\|\widehat\btheta(0)\big\|_2^2 \le b_2$.
Using the Lipschitz property of $\varphi$ concludes the proof.
\end{proof}

\subsection{Approximation with a Huber loss}
Let us fix $\lambda >0$ throughout this section.
For $\rho\in (1,\infty)$, define the Huber loss
\begin{equation}
 \ell_\rho(t) := \begin{cases}
                  t^2 & |t| \le \rho\\
                  \rho(2|t| - \rho)& |t| > \rho
                 \end{cases}
\end{equation}
and the associated problem and objective
\begin{equation}
 \widehat F^{\rm hub}_l(\bD ; \rho, \lambda) := \min_{\btheta \in S_l} L^{\rm hub}(\bD, \btheta; \rho, \lambda)
 \quad\quad
L^{\rm{hub}}(\bD, \btheta;\rho, \lambda) :=
\frac1n \sum_{i=1}^n \ell_\rho\left((\kappa - y_i \bd_i^\sT \btheta)_+ \right) 
+ \frac\lambda2\norm{\btheta}_2^2.
\end{equation}

Here, we show that we can reduce the problem of showing universality of $\widehat F_l^\reg$ to showing universality of $\widehat F_l^\hub$. Namely, we establish the following lemma.
\begin{lemma}
\label{lemma:huber}
For $l\in\{1,2,3\}$,  we have 
\begin{equation}
 \lim_{\rho \to \infty}\lim_{n\to\infty} \left|
\E\left[
\varphi\left(\widehat F_l^{\rm hub}(\bD; \rho, \lambda)\right)
\right] 
-
\E\left[
\varphi\left( \widehat F_l^{\rm reg}(\bD; \lambda)\right)
\right] 
 \right| =0
\end{equation}
for any bounded Lipschitz function $\varphi$.
\end{lemma}

In what follows we suppress $\bD, \lambda$ in the notation for $L^{\rm hub}, \widehat F_l^{\rm hub}, L^{\rm reg}, \widehat F_l^{\rm reg}$.
Define the leave-one-out objective
\begin{equation}
L^{\hub, \up{1}}(\btheta;\rho) :=   L^{\hub}(\btheta;\rho)  - 
 \frac1n\ell_\rho\big(
(\kappa - y_1 \bd_1^\sT\btheta)_+
 \big)
\end{equation}
and let
\begin{equation}
 \widehat\btheta(\rho) := \argmin_{\btheta\in \cS_l} L^{\hub}(\btheta;\rho),
 \quad
 \widehat\btheta^\up{1}(\rho) := \argmin_{\btheta\in  \cS_l } \widehat L^{\hub,\up{1}}(\btheta;\rho),
\end{equation}
%
and define the event
 $\cG := \left\{\norm{\bd}_2 \le 2\sqrt{n}\right\}.$
We have the following auxiliary lemma. 
\begin{lemma}
\label{lemma:loo_upper_bound}
There exist constants $C_0(\lambda),C_1(\lambda,\kappa)>0$ depending only on $\lambda,\kappa$ such that
\begin{equation}
 \big|\bd_1^\sT \widehat\btheta(\rho)\big|\one_{\cG} \le 
 C_0(\lambda)\big|\bd_1^\sT \widehat\btheta_\up{1}(\rho)\big|\one_{\cG} 
  + C_1(\lambda,\kappa)\one_{\cG}.
\end{equation}
\end{lemma}

\begin{proof}
First, note that the KKT conditions and complementary slackness at $\widehat \btheta_\up{1}(\rho)$ give
\begin{equation}
 \grad L^{\hub,\up{1}}\left(\widehat\btheta_\up{1}(\rho);\rho\right) + 
 \eta \left(\grad \pi_l(\widehat\btheta_\up{1}(\rho) ) \right)  + 2\mu \widehat\btheta_\up{1}(\rho) = 0
 ,
 \;
 \eta \left( \pi_l(\widehat \btheta_\up{1}(\rho)) - b_1 \right) = 0,
 \;
 \mu\left( \norm{\widehat\btheta_\up{1}(\rho)}_2^2 - b_2\right) = 0
\end{equation}
for some $\eta,\mu \ge 0$.
Hence, we have
\begin{align}
 \grad L^{\hub,\up{1}}\left(\widehat\btheta_\up{1}(\rho);\rho\right)^\sT
 \left(\widehat\btheta(\rho) - \widehat\btheta_\up{1}(\rho)  \right) 
 &= \eta\left(\widehat\btheta_\up{1} (\rho)
 - \widehat\btheta(\rho) \right)^\sT\left( \grad \pi_l(\widehat\btheta_\up{1}(\rho)) \right)
+
 2\mu\left(\widehat\btheta_\up{1}(\rho)
 - \widehat\btheta(\rho) \right)^\sT \widehat\btheta_\up{1}(\rho)
 \\
 &\ge 
 \eta\left(\pi_l(\widehat\btheta_\up{1}(\rho)) - \pi_l(\widehat\btheta(\rho)) \right)
 + \mu \left(\norm{\widehat\btheta_\up{1}(\rho)}_2^2 -  \norm{\widehat\btheta(\rho)}_2^2\right)
\\
 &= 
 \eta\left( b_1
 -  
 \pi_l(\widehat\btheta_\rho)
 \right)
 + \mu \left(b_2 - \norm{\widehat \btheta(\rho)}_2^2\right)
 \\
 &\ge 0
\end{align}
since $\pi_l(\widehat \btheta(\rho)) \le b_1$, $\norm{\widehat \btheta(\rho)}_2^2 \le b_2$  and $\pi_l(\btheta)$ is convex on $S_l$.
Therefore, by strong convexity of $L^{\hub,\up{1}}(\btheta;\rho)$ in $\btheta$, we have
\begin{align}
\label{eq:LB_huber_loo}
 L^{\hub, \up{1}}(\widehat\btheta(\rho),;\rho) - 
 L^{\hub, \up{1}}(\widehat\btheta_\up{1}(\rho);\rho)
 &\ge \grad L^{\hub, \up{1}}\left(\widehat\btheta_\up{1}(\rho);\rho\right)^\sT
 \left(\widehat\btheta(\rho) - \widehat\btheta_\up{1}(\rho)  \right) 
 + \frac{\lambda}{2} \norm{\widehat\btheta(\rho) - \widehat\btheta_\up{1}(\rho)}_2^2\\
 &\ge 
  \frac{\lambda}{2} \norm{\widehat\btheta(\rho) - \widehat\btheta_\up{1}(\rho)}_2^2.
\end{align}

Now let us bound the left-hand side of~\eqref{eq:LB_huber_loo}. Note that
\begin{align}
 L^{\hub, \up{1}}(\widehat\btheta(\rho);\rho) +
 \frac1n\ell_\rho\big(
(\kappa - y_1 \bd_1^\sT\widehat\btheta(\rho))_+
 \big)
 &=
 L^{\hub,\up{1}}(\widehat\btheta_\up{1}(\rho);\rho) +
 \frac1n\ell_\rho\big(
(\kappa - y_1 \bd_1^\sT\widehat\btheta_\up{1}(\rho))_+
 \big),
\end{align}
so that
\begin{align}
L^{\hub,\up{1}}(\widehat\btheta(\rho);\rho) -
 L^{\hub,\up{1}}(\widehat\btheta_\up{1}(\rho);\rho) 
 &\le
 \frac1n\big(
(\kappa - y_1 \bd_1^\sT\widehat\btheta_\up{1}(\rho))_+
 \big)^2
\end{align}
using that $0 \le \ell_\rho(t) \le t^2$ for all $t$.
Combining with~\eqref{eq:LB_huber_loo}, we conclude that
\begin{equation}
 \norm{\widehat\btheta(\rho) - \widehat\btheta_\up{1}(\rho)}_2 \le \sqrt{\frac{2}{\lambda n}}
 \big(\kappa - y_1 \bd_1^\sT\widehat\btheta_\up{1}(\rho)\big)_+.
\end{equation}

Hence, we can establish the lemma as
\begin{align}
 \big|\bd_1^\sT\widehat\btheta(\rho)\big|
 \one_\cG
 &\le 
 \big|\bd_1^\sT\widehat\btheta_\up{1}(\rho)\big|
 \one_\cG
 +
 \sqrt{\frac{2}{\lambda n}}\norm{\bd_1}_2 \left(\kappa - y_1 \bd_1^\sT\widehat\btheta_\up{1}(\rho)\right)_+
 \one_\cG
 \le
 \big|\bd_1^\sT\widehat\btheta_\up{1}(\rho)\big|
 \one_\cG \left( 1 + 2\sqrt{\frac2\lambda } \right) 
 + 2\sqrt{\frac{2}{\lambda}} \kappa \one_{\cG}.
\end{align}
\end{proof}

We are now ready to prove Lemma~\ref{lemma:huber}.
\begin{proof}[Proof of Lemma~\ref{lemma:huber}]
Let $\widehat\btheta^\reg$ be the minimzer of the problem with the objective $L^\reg$.
First note that we have
\begin{equation}
 L^{\hub}(\widehat\btheta(\rho) ;\rho) \le 
 L^{\hub}(\widehat\btheta_\reg;\rho) \stackrel{(a)}\le
 L^{\reg}(\widehat\btheta_\reg)
 \le  L^{\reg}(\widehat \btheta(\rho))
\end{equation}
where $(a)$ follows from $0 \le \ell_\rho(t)  \le t^2$ for $\rho\in(1,\infty)$ and $t\in\R$.
%
Now taking $\rho \ge \kappa \vee 1$ we have
\begin{align}
 \left|L^{\hub}(\widehat\btheta(\rho);\rho) 
 - L^{\reg}(\widehat\btheta^\reg)\right| 
 &= 
 L^{\reg}(\widehat\btheta^\reg)
 -
 L^{\hub}(\widehat\btheta(\rho) ;\rho)\\
 &\le 
 L^{\reg}(\widehat\btheta(\rho))
 -
 L^{\hub}(\widehat\btheta(\rho) ;\rho)\\
 &= 
 %\sup_{|s|\le M}\frac1n \sum_{i=1}^n\left[ \left(\kappa - s\right)_+^2
 %-
 %\ell_\rho\left(\left(\kappa - s\right)_+\right)
 %\right]\one_{\left\{\left|y_i\bd_i^\sT\widehat\btheta_\rho\right|\le \rho \right\}}\\
 %&\hspace{10mm}+ 
 \frac1n \sum_{i=1}^n \left(\kappa - y_i \bd_i^\sT\widehat\btheta_\rho\right)_+^2
 \one_{\left\{y_i\bd_i^\sT\widehat\btheta(\rho)\le \kappa - \rho \right\}}\\
 &\le
 \frac1n \sum_{i=1}^n \left(\kappa - y_i \bd_i^\sT\widehat\btheta(\rho)\right)_+^2
 \one_{\left\{|y_i\bd_i^\sT\widehat\btheta(\rho)|\ge \kappa + \rho \right\}}\\
 &\le
 %\left|\left(\kappa + M\right)^2 - \ell_\rho\left(\kappa + M\right) \right|\\
 %&\hspace{10mm} +
 \frac4n \sum_{i=1}^n \left|\bd_i^\sT\widehat\btheta(\rho)\right|^2
 \one_{\left\{\left|\bd_i^\sT\widehat\btheta(\rho)\right|> \rho \right\}}.
\end{align}
Here we used that
\begin{equation}
 (\kappa - t)_+ > \rho \textrm{ if and only if }  t \le  -(\kappa + \rho)
\end{equation}
for $\rho \ge \kappa$.
Taking expectations, we have
\begin{align}
 \E\left[
 \left|L^{\hub}(\widehat\btheta(\rho);\rho) 
 - L^{\reg}(\widehat\btheta^\reg)\right| 
 \right] & \le 
  4 \E\left[\left|\bd_1^\sT\widehat\btheta(\rho)\right|^2
 \one_{\left\{\left|\bd_1^\sT\widehat\btheta(\rho)\right|> \rho \right\}}\one_{\cG}\right]
 +
 C_2 n e^{-c_2 n}
 \label{eq:loo_huber_E_loo}
\end{align}
where we used that $\P(\cG^c) \le e^{-c_2 n}$. Now by Lemma~\ref{lemma:loo_upper_bound},
\begin{equation}
 \left\{|\bd_1^\sT \widehat\btheta(\rho)| > \rho\right\}\cap \cG
 \subseteq
\left\{|\bd_1^\sT \widehat\btheta_\up{1}(\rho)|  > \frac{\rho - C_1(\lambda,\kappa) }{C_0(\lambda)}\right\}\cap \cG \\
\end{equation}
and
\begin{equation}
 4|\bd_1^\sT \widehat\btheta(\rho)|^2\one_\cG
 \le C_3(\lambda) |\bd_1^\sT \widehat\btheta_\up{1}(\rho)|^2 \one_\cG + C_4(\lambda,\kappa)\one_\cG
 =: P(\bd_1^\sT\widehat\btheta_\up{1}(\rho); \lambda,\kappa)\one_\cG
\end{equation}
so letting $\cB:=\{\norm{\bW}_\op \le C\}$, 
can bound the term in~\eqref{loo_huber_E_loo} as
\begin{align}
4 \E\left[\left|\bd_1^\sT\widehat\btheta(\rho)\right|^2
 \one_{\left\{\left|\bd_1^\sT\widehat\btheta(\rho)\right|> \rho \right\}}\one_{\cG}\one_\cB \Big| \bW\right]
 &\le \E\left[
 P(\bd_1^\sT\widehat\btheta_\up{1}(\rho); \lambda,\kappa) 
 \one_{\left\{\left|\bd_1^\sT\widehat\btheta_\up{1}(\rho)\right|> (\rho-C_0(\lambda))/C_1(\lambda,\kappa) \right\}}
 \one_\cB \Big| \bW
 \right]\\
 &\le \E\left[
 C_4 P(\bd_1^\sT\widehat\btheta_\up{1}(\rho); \lambda,\kappa)^2\one_\cB\Big| \bW
 \right]^{1/2} \P\left(
 \left|\bd_1^\sT\widehat\btheta_\up{1}(\rho)\right|> (\rho-C_0(\lambda))/C_1(\lambda,\kappa)
 |
 \right)\\
 &\le 
 C_5(\lambda,\kappa) e^{-c_4 (\rho - C_0(\lambda))/C_1(\lambda,\kappa)}
\end{align}
where the last equality follows since
since $\widehat\btheta_\up{1}(\rho)$ 
is independent of the $\cO(1)$-subgaussian
$\bd_1$ and $P^2$ is polynomial in this subgaussian variable.
Combining, we conclude that
\begin{align}
 &\left|
\E\left[
\varphi\left( \min_{\btheta\in S_c}L^{\hub}(\btheta;\rho,\lambda)\right)
\right] 
-
\E\left[
\varphi\left( \min_{\btheta\in S_c}L^{\hub} (\btheta;\infty,\lambda)\right)
\right] 
 \right| \\
 &\hspace{20mm}\le \norm{\varphi}_\Lip
 \left(
  C_2 n e^{-c_2 n} + 
 C_5(\lambda,\kappa) e^{-c_4 (\rho - C_0(\lambda))/C_1(\lambda,\kappa)}
 \right).
\end{align}
Taking $n\to\infty$ then $\rho \to\infty$ concludes the proof.



\end{proof}

\subsection{Infinity norm bound on minimizer}
Here, we establish that the minimizer 
of the objective 
$ L^\hub(\bD, \btheta;\rho,\lambda)$ 
over the set $\cS_l$, for fixed $\rho\in(1,\infty),\lambda>0$  and $l\in\{1,2,3\}$ 
has a small $\ell_\infty$ norm with high probability.


Namely, we establish the following lemma.
\begin{lemma}
\label{lemma:inf_norm_surrogate}
Let $\widehat\btheta$ be the minimizer of $L^{\hub}(\bD, \btheta; \rho, \lambda)$. Then under the assumptions of Theorem~\ref{thm:univ_fixed_kappa}, we have
\begin{equation}
 \norm{\widehat \btheta}_\infty \le C_4(\rho,\lambda)\frac{\log p}{\sqrt{p}} +  C_7 (b_1, b_2, \rho, \lambda) n^{-\delta}
\end{equation}
with probability larger than
$1 - C_2 \exp\{-c (\log p)^2\}$.
\end{lemma}



We do this via a leave-one-out approach.
%
Fix a column index $j\in[p]$.
For $\btheta\in\R^p$, let $\btheta_{\up{j}}(t)$ be the vector obtained by replacing the $j$th element of $\btheta$ with $t$.
Similarly, let $\bd_{i,\up{j}} := \bd_{i,\up{j}}(0)$ be the vector $\bd_i$ with its $j$th element set to $0$.

To simplify notation, let us use $L$ in place of $L^{\hub}$, suppressing some of its arguments. Namely, we have
\begin{equation}
L(\btheta_\up{j}(t)):= \frac1n \sum_{i=1}^n 
\ell\left(\bd_{i,\up{j}(0)}^\sT \btheta_\up{j}(0) + d_{i,j}t; y_i \right)+ \frac{\lambda}{2} \norm{\btheta_\up{j}(0)}_2^2 + \frac\lambda2 t^2
\end{equation}
for $\btheta\in\R^p$ and $t\in\R$;
here we defined
$ \ell(s;y) := \ell_\rho\big((\kappa - y s)_+\big).$

For fixed $t \in \R$, let
\begin{equation}
 \widehat \btheta_{\up{j},t}:= \argmin_{ \btheta\in \cS_l, \theta_j = t}  L(\btheta).
\end{equation}

We remark that $\ell$ is convex since $\ell_\rho$ restricted to $R_{>0}$ is non-decreasing.
Furthermore, the constraint set is convex in $\btheta_{\up{j}}(0)$ for a fixed $t$ since $\cS_l$ was convex.
The convexity of $\ell(s;y)$ and strong convexity of the norm squared
at $\widehat \btheta_\up{j},0$ imply that for all $\btheta\in\cS_l$ we have
\begin{align}
 L(\btheta) &\ge
 \frac1n \sum_{i=1}^n
\ell(\widehat\btheta_{\up{j},0}^\sT\bd_{i,\up{j}}(0);y_i) 
+ \frac1n\sum_{i=1}^n\ell'(\widehat\btheta_{\up{j},0}^\sT\bd_{i,\up{j}}(0);y_i) \left( \btheta -\widehat \btheta_{\up{j},0}\right)^\sT \bd_{i,\up{j}}(0) +  
\frac\lambda2\norm{\widehat\btheta_{\up{j},0}}_2^2  \\
&+ \frac1n\sum_{i=1}^n\ell'(\widehat\btheta_{\up{j},0}^\sT \bd_{i,\up{j}}(0);y_i)\theta_{j} d_{i,j}
+\frac\lambda2 |\theta_{j}|^2
 + \lambda\left(\btheta- \widehat\btheta_{\up{j},0}\right)^\sT\widehat\btheta_{\up{j},0}
 + \frac\lambda2 \norm{\btheta_\up{j}(0) - \widehat\btheta_{\up{j},0}}_2^2\\
&= L(\widehat \btheta_{\up{j},0}) + \widehat D \theta_{i,j} + \frac\lambda2 \theta_{i,j}^2 
+ \frac1n \sum_{i=1}^n\ell'(\widehat\btheta_{\up{j},0}^\sT\bd_{i,\up{j}}(0);y_i) \left( \btheta -\widehat\btheta_{\up{j},0}\right)^\sT \bd_{i,\up{j}}(0)\\
&+ \lambda\left(\btheta - \widehat\btheta_{\up{j},0}\right)^\sT\widehat\btheta_{\up{j},0}
+ \frac{\lambda}2 \norm{\btheta_\up{j}(0) - \widehat\btheta_{\up{j},0}}_2^2.
\label{eq:lower_bound_loo}
\end{align}
where we defined $\widehat D_j:= \sum_{i=1}^n \ell'(\widehat\btheta_{\up{j},0}\bd_{i,\up{j}}(0);y_i)d_{i,j} / n$.

We would like to assert that $L(\btheta)$ is at least  $L(\widehat \btheta_{\up{j},0}) + \widehat D_j  \theta_{i,j} + \frac\lambda2 \theta_{i,j}^2$,
up to some error term.
This, in turn, gives a bound on $t$ in terms of $\widehat D_j$. We do this in the following lemma.

\begin{lemma}
Let $\widehat \theta_{j}$ be the $j$th coordinate of the minimizer of $L(\theta)$. Then
for $l\in\{1,2,3\}$, we have
\begin{equation}
 |\widehat \theta_j| \le \frac{2 \widehat D_j }{\lambda} + \frac{2}\lambda \left( \frac{2\rho}{\sqrt{n}} \norm{\bD}_\op + \lambda b_2\right)^{1/2}C(b_1)^{1/2} \norm{\bSigma\btheta^\star}_\infty^{1/2}.
\end{equation}
for some $C >0$ depending only on $b_1$.
\end{lemma}

\begin{proof}

First, note that the KKT conditions for $\widehat\btheta_{\up{j},0}$ along with complementary slackness imply that
%\begin{align}
% \frac1n \sum_{i=1}^n \ell'(\widehat\btau_0^\sT\ba_i; y_i)\ba_i + \delta\widehat\btau_0 + \lambda \grad g_c(\widehat\btau_0) + 2 \mu \norm{\widehat\btau_0}=0
%\end{align}
%\begin{equation}
% \lambda\left(G({\widehat\btau_0}) - L\right) = 0
%\end{equation}
%for some $\lambda >0$. Hence, we have for any $\btheta$ with $\norm{\btheta}_2\le1$
\begin{align}
\label{eq:kkt_lower_bound_loo}
h(\btheta) := \frac1n \sum_{i=1}^n \ell'(\widehat\btheta_{\up{j},0}^\sT\bd_{i,\up{j}}(0);y_i)\bd_{i,\up{j}}(0)^\sT(\btheta - \widehat\btheta_{\up{j},0})  
+ \lambda\widehat\btheta_{\up{j},0}^\sT(\btheta -\widehat\btheta_{\up{j},0}) 
&\ge 0
\end{align}
for all $\btheta \in\cS_l$.

For $l\in\{2,3\}$, note that $\cS_l$ is orthosymmetric: indeed, if $\btheta \in\cS_l$, then $\btheta_{\up{j}}(-\theta_{j}) \in\cS_l$ directly from the definition. By convexity, we then have that
$\btheta_{\up{j}}(0)\in\cS_l$.
Hence, using the lower bound in~\eqref{eq:lower_bound_loo} and the KKT lower bound in~\eqref{eq:kkt_lower_bound_loo}, we have, for any $\btheta \in \cS_l$,
\begin{equation}
 L(\widehat\btheta_{\up{j},0}, 0) \ge L(\btheta) \ge 
 L(\widehat\btheta_{\up{j},0}, 0) + \widehat D \theta_{j} + \frac\lambda2 \theta_{j}^2.
\end{equation}
Minimizing over $\btheta \in\cS_l$ gives, after cancellations
\begin{equation}
 | \widehat \theta_j | \le \frac{2\widehat D}{\lambda}
\end{equation}
as desired.

For the case of $l=1$, $\cS_l$ lacks orthosymmetry. Hence, we instead show that $(\btheta)$ will be ``approximately in'' $\cS_l$.
Namely, Lemma~\ref{lemma..} below establishes that for any $\btheta \in\cS_1$, 
there exists some $\overline \btheta$ such that $\overline\btheta_{\up{j}}(0) \in\cS_l$ and 
\begin{equation}
 \norm{\btheta_\up{j}(0) - \overline \btheta_\up{j}(0) }_2 \le C(b_1) \norm{\Sigma \btheta^\star}_\infty
\end{equation}
where $C(b_1) >0$ is some constant depending only on $b_1$.
Using linearity of $h(\btheta)$, $h(\overline\btheta_\up{j}(0)) \ge 0$ and that
\begin{equation}
 \norm{\grad h(\btheta)}_2 \le \norm{\frac1n \sum_{i=1}  \ell'(\widehat\btheta_{\up{j},0}^\sT\bd_{i,\up{j}}(0);y_i)\bd_{i,\up{j}}(0)}_2
+ \lambda\norm{\widehat\btheta_{\up{j},0}}_2 \le \frac1n \norm{\bD}_\op\norm{\ba}_2 + \lambda \norm{\widehat\btheta_{\up{j},0}}_2,
\end{equation}
for $\ba\in\R^n$ with $|a_i| = |\ell'(\widehat\btheta_{\up{j},0}^\sT \bd_{i,\up{j}}(0); y_i)| \le 2\rho$, we have 

\begin{equation}
 h(\btheta) \ge - \left( \frac{2\rho}{\sqrt{n}} \norm{\bD}_\op + \lambda b_2\right)C(b_1) \norm{\bSigma\btheta^\star}_\infty.
\end{equation}
Combing this lower bound with~\eqref{eq:lower_bound_loo} and optimizing over $\btheta\in\cS_1$ yields
\begin{equation}
0 \ge \widehat D \widehat\theta_{j} + \frac{\lambda}2 \widehat\theta_{j}^2 - \left( \frac{2\rho}{\sqrt{n}} \norm{\bD}_\op + \lambda b_2\right)C(b_1) \norm{\bSigma\btheta^\star}_\infty.
\end{equation}
Hence, we have
\begin{equation}
 |\widehat \theta_j| \le \frac{2 \widehat D }{\lambda} + \frac{2}\lambda \left( \frac{2\rho}{\sqrt{n}} \norm{\bD}_\op + \lambda b_2\right)^{1/2}C(b_1)^{1/2} \norm{\bSigma\btheta^\star}_\infty^{1/2}.
\end{equation}

\end{proof}


\begin{lemma}
Fix any $j\in[p]$.
For any $\btheta \in\cS_1$, there exists some $\overline \btheta \in\cS_l$ such that $\overline\btheta_j = 0$
and
\begin{equation}
 \norm{\overline \btheta - \btheta_\up{j}}_2 \le C(b_1) \norm{\Sigma \btheta^\star}_\infty
\end{equation}
where $C(b_1) >0$ is some constant depending only on $b_1$.
\end{lemma}


\begin{proof}
Recall the definition of $\cS_1$:
\begin{equation} 
 \cS_1 := \{\norm{\btheta}_2^2 + s \btheta^\sT\bSigma \btheta^\star  \le b_1, \norm{\btheta}_2^2 \le b_2(1, b_1)\}
 \end{equation}
 and note that the ellipsoid constraint implies
 \begin{equation}
  \norm{\btheta}_2^2  \le b_1 + |s| \norm{\btheta}_2 \norm{\bSigma}_\op \norm{\btheta^\star}.
 \end{equation}
 This puts the constraint
 \begin{equation}
  \norm{\btheta}_2^2 \le \frac{s_0 + \sqrt{s_0^2\oslambda^2 \norm{\btheta^\star}_2^2 + 4 b_1}}{2}
 \end{equation}
 on the norm. In other words, the explicit constraint on the norm of $\btheta$ in the definition of $\cS_1$ can be ignored. 
 So we can write
 \begin{equation}
 \cS_1 = \{\norm{\btheta}_2^2 - 2 \btheta^\sT \bv_s + \norm{\bv_s}_2^2 \le b_1(s)\} =  \{\norm{\btheta - \bv_s}_2^2 \le b_1(s)\}.
\end{equation}
Here, we defined 
\begin{equation}
 \bv :=  -\frac{s}{2}  \bSigma\btheta^\star,\quad \widetilde b_1 := b_1 + \norm{\bv_s}_2^2.
\end{equation}

Now let $\widetilde\btheta \in \cS_1$. If $\widetilde \btheta_\up{j} \in \cS_1$, we are done so assume $\widetilde \btheta_\up{j} \not\in \cS_1$. 
First, we note that $\bv \in S_1$. Furthermore, 
\begin{equation}
 \norm{\bv - \bv_{\up{j}}}_2^2 \le \norm{\bv}_\infty^2 \le \norm{\bv}_2^2 + b_1 = \widetilde b_1.
\end{equation}
Hence, we also have $\bv_\up{j} \in \cS_1$.
Now let 
\begin{equation}
 \overline \btheta := \argmin_{ \{\btheta \in \cS_1:\exists c \textrm{ s.t. } \btheta = \bv_\up{j}+ c(\widetilde \btheta_\up{j} - \bv_\up{j})\} }  \norm{\btheta - \widetilde\btheta_\up{j}}_2^2.
\end{equation}
(The minimum is achieved and unique since $\cS_1$ is closed and convex.)
Clearly, $\overline \btheta = \overline\btheta_\up{j}$ and $\norm{\overline\btheta_\up{j} - \bv}_2 = \widetilde b_1$ since $\widetilde \btheta_\up{j} \not\in\cS_1$.
Now by Pythagoras',
\begin{align}
 \norm{\overline\btheta_\up{j} - \widetilde\btheta_\up{j}}_2^2 &= (1-c)^2 \norm{\bv_\up{j} - \widetilde \btheta_\up{j}}_2^2
 = (1-c)^2 \left( \norm{\bv - \widetilde\btheta_\up{j}}_2^2 - \norm{\bv - \bv_\up{j}}_2^2\right)
 \le (1-c)^2 \norm{\bv - \widetilde\btheta_\up{j}}_2^2.
\end{align}

We can upper bound the norm squared term in the previous display by
\begin{align}
\norm{\widetilde\btheta_\up{j} - \bv}_2^2 &= \norm{\widetilde\btheta  - \bv}_2^2 - \theta_j^2 + 2 \theta_j v_j \le \widetilde b_1 + 2 b_2^{1/2} \norm{\bv}_\infty.
\label{eq:upper_bound_orth_proj}
\end{align}
since $\btheta\in \cS_1 \Rightarrow \norm{\btheta}_2 \le 2 b_2^{1/2}$.
Meanwhile, to compute $c$, use Pythagoras' again to obtain
\begin{equation}
 \norm{\bv - \overline\btheta_\up{j}}_2^2 - \norm{\bv - \bv_\up{j}}_2^2 =  \norm{\overline\btheta_\up{j} - \bv_\up{j}}_2^2 = 
 c^2 \norm{\widetilde \btheta_\up{j} - \bv_\up{j}}_2^2 = c^2 \left(\norm{\widetilde\btheta_\up{j} - \bv}_2^2 - \norm{\bv - \bv_\up{j}}_2^2\right).
\end{equation}
Using that
$\norm{\bv - \overline{\btheta}_\up{j}}_2^2  = \widetilde b_1$ gives
\begin{equation}
c = \left(\frac{\widetilde b_1 - \norm{v_j}_2^2}{\norm{\widetilde\btheta_\up{j} - \bv}_2^2 - \norm{v_j}_2^2}\right)^{1/2}.
\end{equation}


So
\begin{align}
 1-c
% &= \frac{\sqrt{\norm{\widetilde\btheta_\up{j}- \bv}_2^2 - {v_j}^2} -\sqrt{\widetilde b_1 - {v_j}^2}}{\sqrt{\norm{\widetilde\btheta_\up{j} - \bv}_2^2 - {v_j}^2}}\\
% &=  \frac{\norm{\widetilde\btheta_\up{j} - \bv}_2^2  -\widetilde b_1}{\left(\sqrt{\norm{\widetilde\btheta_\up{j} - \bv}_2^2 - {v_j}^2}\right)
%\left(
%\sqrt{\norm{\widetilde\btheta_\up{j} - \bv}_2^2 - v_j^2} +\sqrt{\widetilde b_1 - v_j^2}
%\right) 
% }\\
 &\stackrel{(a)}\le \frac{\norm{\widetilde\btheta_\up{j} - \bv}_2^2  -\widetilde b_1}{\left(\sqrt{\widetilde b_1 - v_j^2}\right)
\left(
\sqrt{\widetilde b_1 - v_j^2} +\sqrt{\widetilde b_1 - v_j^2}
\right) 
 }
 \stackrel{(b)}\le \frac{2b_2^{1/2} \norm{\bv}_\infty}
 {2\left(\widetilde b_1 - \norm{\bv}_\infty^2\right)
 }
 \stackrel{(c)}\le \frac{b_2^{1/2}}{b_1} \norm{\bv}_\infty,
\end{align}
where $(a)$ follows from $\norm{\widetilde\btheta_\up{j} - \bv}_2^2 \ge \widetilde b_1$ since $\widetilde\btheta_\up{j} \not\in \cS_1$ and 
$(b)$ follows from the upper bound
derived in~\eqref{eq:upper_bound_orth_proj}, and in $(c)$ we used that $ \widetilde b_1 - \norm{\bv}_\infty^2 \ge  b_1$.
%
Hence,
\begin{equation}
 \norm{\overline\btheta_\up{j} - \widetilde\btheta_\up{j}}_2^2 \le \frac{b_2^{1/2}}{b_1} \norm{\bv}^2_\infty \left(\widetilde b_1 + 2b_2^{1/2} \norm{\bv}_\infty\right) \le  
 C(b_1) \norm{\bv}_\infty^2
\end{equation}
for some $C >0$.


\end{proof}

Let 
\begin{equation}
 \cG := \left\{ \norm{\bZ}_\op\le \frac{2}{\sqrt{n}} \right\}.
\end{equation}
Note that
$$\widehat D_j:= \frac1n\sum_{i=1}^n \ell'(\widehat\btheta_{\up{j},0}\bd_{i,\up{j}}(0);y_i)d_{i,j} = \frac1n \ba_j^\sT \widetilde\bd_j$$
for $\ba_j \in \R^n$, and $\widetilde\bd_j$ the $j$th column of $\bD$. Conditional on fixed $\bZ\in\cG$, $\ba_j$ is independent of $\widetilde \bd_j$ for all $j$ since $y_i$ is only a function of the $j$th 
weight $\bw_j$. Then since $\norm{\ba_j}_\infty \le 2 \rho$, we have that each $\widehat D_j$ is $2\rho/\sqrt{n}$ subgaussian. Hence,

So
\begin{equation}
 \P\left(\left\{\max_{j\le p } \widehat D_j \ge 2\rho \frac{\log{p}}{\sqrt{p}}\right\} \right) \le C_1 \exp\left\{-c (\log p)^2\right\} + \P(\cG^c)  \le C_2 \exp\{-c (\log p)^2\}.
\end{equation}

Hence, by Lemma~\ref{lemma..}, we have
\begin{equation}
\P\left(\norm{\widehat \btheta}_\infty \ge \frac{4 \rho}{\lambda} \frac{\log p}{\sqrt{p}}  +
\frac{2}\lambda \left( \frac{2\rho}{\sqrt{n}} \norm{\bD}_\op + \lambda b_2\right)^{1/2}C(b_1)^{1/2} \norm{\bSigma\btheta^\star}_\infty^{1/2} \right)
\le C_2 \exp\{-c (\log p)^2\}.
\end{equation}
Using that $\norm{\bD}_\op \le C_2/\sqrt{n}$ with probability at least $1- C_3 e^{-c_2 n}$ and that $\norm{\bSigma \btheta^\star}_\infty \le C^6 n^{-\delta}$ for some $\delta>0$,
we conclude that 
\begin{equation}
 \norm{\widehat \btheta}_\infty \le C_4(\rho,\lambda)\frac{\log p}{\sqrt{p}} +  C_7 (b_1, b_2, \rho, \lambda) n^{-\delta}
\end{equation}
with probability larger than
$1 - C_2 \exp\{-c (\log p)^2\}$.




\subsection{Pointwise-Gaussianity of the random features model}
In this section, we provide a standalone proof of the Pointwise Gaussianity of the random features model. We note that this result was apriori established in \notate{Cite the physicists} then in
\notate{Cite hulu}.
Let us define augmented features
\begin{equation}
  \bxi_i := (\bx_i^\sT ,\bz_i^\sT )^\sT \in \R^{p + d}\quad
   \bgamma_i := (\bg_i^\sT ,\bz_i^\sT )^\sT \in \R^{p + d}.
 \end{equation}
We prove the following lemma.

\begin{lemma}
Let $\delta_n$ be any sequence such that $\delta_n\to0$. Then
any bounded Lipschitz function $\varphi$, we have
 \begin{equation}
  \lim_{n\to\infty} \sup_{\norm{\bzeta_1}_\infty \le \delta_n, \norm{\bzeta}_2 \le C}
  \left|
  \E[\varphi( \bzeta^\sT\bxi) ]
  -\E[\varphi( \bzeta^\sT\bgamma) ]
  \right|=0.
 \end{equation}
\end{lemma}
\begin{proof}
Let us write $\bzeta = (\bzeta_1^\sT,\bzeta_2^\sT)^\sT$ for 
$\bzeta_1 \in\R^p, \bzeta_2\in\R^d$ and define
 
$$h(\bz) := \zeta^\sT \bxi(\bz)= \sum_{j=1}^p\xi_j \sigma(\bw_j^\sT \bz) + \sum_{j=p+1}^{p+d} \xi_jz_j.$$

We compute the derivatives of $h(\bz)$:
\begin{align}
 \grad h(\bz) = \bW^\sT \bM_1 \bzeta_1 + \bzeta_2\quad
\grad^2 h(\bz) =  \bW^\sT \bM_2 \diag\{\bzeta_1\} \bW.
\end{align}

So by the second order Poincar\'e inequality, we have
\begin{equation}
  \left|
  \E[\varphi( \bzeta^\sT\bxi)|\bW ]
  -\E[\varphi( \bzeta^\sT\balpha)|\bW ]
  \right| \le  C \frac{\left(\norm{\bW}_\op \norm{\sigma'}_\infty \norm{\bzeta_1}_2 + \norm{\bzeta_2}_2 \right)
  (\norm{\bW}_\op^2 \norm{\sigma''}_\infty \norm{\bzeta_1}_\infty)}{\Var(\bzeta^\sT\bxi)}
\end{equation}
where $\balpha$ is a Gaussian vector with mean $0$ and covariance matching that of $\bxi$.
So for any $\delta>0$, we have
\begin{equation}
 \sup_{\norm{\bzeta_1}_\infty \le \delta_n, \norm{\bzeta}\le C,\Var(\bzeta^\sT\bxi) > \delta} 
  \left|
  \E[\varphi( \bzeta^\sT\bxi)|\bW ]
  -\E[\varphi( \bzeta^\sT\balpha)|\bW ]
  \right| \le  C_1 \frac{\norm{\bW}_\op^3 \delta_n}{\delta} 
\end{equation}
Meanwhile, 
\begin{equation}
 \sup_{\Var(\bzeta^\sT\bxi) \le \delta} 
  \left|
  \E[\varphi( \bzeta^\sT\bxi) ]
  -\E[\varphi( \bzeta^\sT\balpha) ]
  \right|  
  \le C_2 \norm{\varphi}_\Lip \Var(\bzeta^\sT \bxi)^{1/2} \le C_3 \delta^{1/2}.
\end{equation}
Since $\norm{\bW}_\op \le C_4$ with probability at least $1-e^{-c_0 p}$, we have

\begin{align}
 \sup_{
 \norm{\bzeta_1}_\infty \le \delta_n, \norm{\bzeta}_2\le C
 } 
  \left|
  \E[\varphi( \bzeta^\sT\bxi) ]
  -\E[\varphi( \bzeta^\sT\balpha) ]
  \right|  \le
  C_5 \frac{\delta_n}{\delta} + 
   C_3 \delta^{1/2} + \norm{\varphi}_\infty (e^{-c_0 p}).
\end{align}
Sending $n \to\infty$ then $\delta \to 0$ shows that the statement of the lemma holds with $\bgamma$ replaced with $\balpha$.
Now by HuLu20, we have
\begin{equation}
 \lim_{n\to\infty}\norm{\Cov(\balpha | \bW)- \Cov(\bgamma|\bW) }_\op  = 0
\end{equation}
for $\norm{\bW}_\op \le C_4$.
Hence,
\begin{equation}
 |\E\left[\varphi(\bzeta^\sT \balpha) - \varphi(\bzeta^\sT\bgamma)\big|\bW\right] |
 \le
\norm{\varphi}_\Lip
\norm{\bzeta}_2^2 \norm{\Cov(\alpha|\bW) - \Cov(\gamma|\bW) }_\op.
\end{equation}
Now using that the bound on $\norm{\bW}_\op$ holds with high probability once again and optimizing over $\bzeta$ then taking $n\to\infty$ completes the proof.








\end{proof}





\subsection{Proof of Theorem}

Let $C_0,c_0,C_1$ and $\delta >0$ be constants such that 
$\norm{\widehat\btheta}_\infty \le C_0 n^{-\delta}$ with probability 
at least $1 - C_1 \exp\{-c_0 (\log p)^2\}$ by Lemma~\ref{lemma:inf_norm_surrogate}. 
Let $\cG$ denote this high probability set.

To put this in the framework of [MS22], let us define new features
\begin{equation}
  \bxi_i := (\bx_i^\sT ,\bz_i^\sT )^\sT \in \R^{p + d}
 \end{equation}
 and new Gaussian features
\begin{equation}
   \bgamma_i := (\bg_i^\sT ,\bz_i^\sT )^\sT \in \R^{p + d}
 \end{equation}
 where $\bg_i$ are the Gaussian equivalent of $\bx_i$. 
 \notate{Need to write these explicitly at some point.}
 Let us use $\bXi$ and $\bGamma$ to denote the feature matrices of these augmented features respectively.
Then the labels can be viewed as a function of 
$ \bxi_i^\sT \bzeta^\star = \bz_i^\sT \bbeta^\star$
where $\bzeta^\star = ({\mathbf 0}^\sT, \bbeta^{\star\sT})^\sT \in \R^{p+d}$. 
Now define the sets
\begin{equation}
\cC_l := \{\bzeta\in\R^{p+d} : \bzeta = (\btheta^\sT, {\mathbf 0}^\sT)^\sT, \btheta\in\cS_l\}  \subseteq \R^{p+d},
\end{equation}
and
\begin{equation}
 \cC_{l,\infty} := \cC_l \cap \{\bzeta \in\R^{p+d}, \norm{\bzeta}_\infty \le C_0 n^{-\delta} \}.
\end{equation}

We verify the assumptions of [MS22] for the problem
\begin{equation}
\widehat F^{\aug}(\bXi,\cC_{l,\infty}):= \min_{\bzeta \in\cC_{l,\infty}} \frac1n \sum_{i=1}^n \ell_\rho\left((\kappa - \bxi_i^\sT \bzeta y_i)_+\right) + \frac{\lambda}2 \norm{\bzeta}_2^2
\quad\P(y_i = +1 | \bxi_i) = f(\xi_i^\sT \bzeta^\star).
\end{equation}

Clearly, $\ell_\rho((\kappa - t s)_+)$ is Lipschitz in $t$ for fixed $s$ and Lipschitz in $s$ for fixed $t$, and $f$ is Pseudo Lipschitz
so Assumption 1 is Satisfied. The sets $\cC_l$ are compact subsets of $\cS_l \otimes \R^d$ so Assumption 2 is satisfied, and for any $\beta^\star$, Assumption 3 is clearly satisfied.
The $\ell^2$ regularization clearly satisfies Assumption 4. Finally, by subgaussianity of $\bx$, and that
\begin{equation}
\lim_{p\to\infty}  \sup_{\bzeta \in\cC_{l,\infty}}\left|\E\left[\varphi(\bzeta^\sT \bxi)\right]- \E\left[\varphi(\bzeta^\sT \bgamma)\right]\right| = 0,
\end{equation}
Assumption 5 is satisfied.
Hence, by Theorem 1 of [MS22], we have,
by first conditioning on $\bW \in\cB := \{\norm{\bW}_\op \le C\}$, 
for any bounded Lipschitz test function $\varphi$
\begin{equation}
 \lim_{n\to\infty} \left| \E\left[\varphi\left(\widehat F^\aug(\bXi) \right)\right]
- 
\E\left[\varphi\left(\widehat F^\aug(\bGamma) \right)\right]
\right| = 0.
\end{equation}
Meanwhile, note that
\begin{align}
|\E[\varphi( \widehat F^\aug(\bXi, \cC_{l}))-\varphi( \widehat F^\aug(\bXi, \cC_{l,\infty}))] |
&\le
\norm{\varphi}_\infty
\P\left(\cG^c\right) \le C_1 \norm{\varphi}_\infty e^{-c_0 (\log p)^2 }.
\end{align}
Combining with Lemmas~\ref{lemma: 1,2,3} gives statement of the Theorem.

%\begin{lemma}
%For all $\varphi$ B-L, we have
%\begin{equation}
%\lim_{p\to\infty}\sup_{\bzeta\in\cC_p} \left|\E\left[\varphi\left( \bzeta^\sT \bxi \right)\Big| \bW \in\cB \right] 
%- \E\left[\varphi\left( \bzeta^\sT\bgamma \right)\Big| \bW\in\cB \right]\right|=0.
%\end{equation}
%\end{lemma}
%
%However, this is a direct consequence of Theorem 2 of [HL20].
%


\section{Deferred proofs}
\begin{lemma}
\label{lemma:S-l_inclusion}
For $l\in\{1,2,3\}$,  $|s| \le s_0$ and $L>0$,
$S_l(s,L)$ is convex and satisfies
\begin{equation}
B_2^p(c(L,R))  \subseteq S_l(s,L,R) \subseteq B_2^p(C(L,R)).
\end{equation}
for constants $c(L,R),C(L,R) >0$ depending only on $L ,R>0$.
\end{lemma}

\begin{proof}
 For $l=1$, note that $\theta \in S_1(s,L)$ implies
 \begin{equation}
  \norm{\btheta}_2^2 - |s| \norm{\btheta}_2 \oslambda\le L
 \end{equation}
 and hence
 \begin{equation}
  \norm{\btheta}_2 \le \frac{|s|\oslambda}{2} + \frac{\sqrt{s^2\oslambda + 4 L}}{2} \le C_0(L) 
 \end{equation}
 for $|s| \le s_0$. Meanwhile,
 letting $c_0(L)$ be the solution $c_0(L)^2 + c_0(L)/2 = L$, 
 if $\norm{\btheta}_2 \le c_0(L)$ then we have
 \begin{equation}
  \norm{\btheta}_2^2 + s C_1(\btheta) \le \norm{\btheta}_2^2 + |s| \oslambda \norm{\btheta}_2  \le c_0(L)^2 + \frac{c_0(L)}{2} = L.
 \end{equation}
Hence we showed that for any $|s| \le s_0$ and $L>0$,
\begin{equation}
     B_2^p(c_0(L)) \subseteq  S_1(s,L) \subseteq B_2^p(C_0(L)).
\end{equation}

For $l=2$, note that $\norm{\btheta}_2^2 + s\norm{\btheta}_\Sigma^2 = \norm{\btheta}_{(\bI + s \bSigma)}^2$ and hence
Since for $|s| \le s_0$ we have 
\begin{equation}
\frac12 \le \sigma_{\min}(\bI + s\bSigma) \le \norm{\bI + s\bSigma}_\op \le 2,
\end{equation}
we conclude that 
\begin{equation}
B_2^p(L/2)  \subseteq S_2(s,L) \subseteq B_2^p(2L).
\end{equation}
Finally, for $l=3$ the upper inclusion follows directly from the definition, while the inner one
follows from $\norm{\btheta}_4^4 \le \norm{\btheta}_2^4$. 
\end{proof}






\section{Margin lower bound}


\subsection{Lower bounding the minimum singular value of sub-matrices of $({{\bf y} \odot {\bf X}})$} 
Let $m =  n / K'$ for some $K'$ to be chosen later.
 Take $M := {n\choose m}$. 
Now let
$\bX_1, \dots, \bX_M$ 
be an enumeration of all $n\choose m$ sub-matrices of $\bX$ 
in $\R^{m\times p}$ obtained by leaving out $n-m$ rows of $\bX$.
For $j\in[M]$, let $\bX_j'\in\R^{(n-m)\times p}$ be the sub-matrix of the remaining rows.

For a constant $c>0$,
define the event
\begin{equation}
 \cT_1 := \left\{\bX : s_{\min}(\bX_j^\sT) \ge c \sqrt{p} \textrm{ for all } j\in[M] \right\},
\end{equation}
and for $C >0$, define
\begin{equation}
\cT_2 := \left\{\bX : \norm{\bX'_j}_\op \le C \sqrt{p} \textrm{ for all } j\in[m]\right\}.
\end{equation}

The goal of this section is to prove that $\cT_1$ and $\cT_2$ are high probability sets.

\subsubsection{Linear transforms of i.i.d.}

\begin{lemma}
Let
$ K' = \left(K( 1 \vee 1/\sgamma) \right)$ for some fixed and sufficiently large $K$.
We have
 \begin{equation}
  \P(\cT_1) \ge 1-C(K)e^{-c(K) p}
 \end{equation}
 for some $C(K),c(K)>0$ depending only on $K$.
\end{lemma}


\begin{lemma}
 There exists some $C(\kappa)>0$ such that 
\begin{equation} 
\lim_{n\to\infty} \P\left(\big\{\widehat H_l^\bD(s,\kappa) < C(\kappa)\big\} \cap \cG \right)  = 1.
\end{equation}
Furthermore, letting $\widehat\btheta_l^\bD(s,\kappa)$ be the associated minimizer, for some $\widetilde C(\kappa)$ depending on $\kappa$
\begin{equation}
 \lim_{n\to\infty} \P\left(\left\{\norm{\widehat\btheta_l^\bD(s,\kappa)}_2< \widetilde C(\kappa)\right\} \cap \cG  \right)
\end{equation}

\end{lemma}
\begin{proof}

 Note that the constraint in the definition of $H_l$ implies 
 \begin{equation}
  \norm{\btheta}_2 \ge \kappa \frac{\sqrt{n}}{\norm{\by \odot\bX}_\op} \ge \frac\kappa{\sfK};
 \end{equation}
recall that $\sK$ satisfies $\norm{\bX}_\op/\sqrt{n} \le \sfK$ w.h.p. Assuming, w.l.o.g. that $\kappa/\sfK <1$ we have for $l=1$
\begin{align}
 \widehat H_1^\bD(s,\kappa) 
 &\stackrel{(a)}\le \min_{y_i\btheta^\sT\bd_i \ge \kappa} \norm{\btheta}_2^2 + \frac12 \norm{\btheta}_2\\
 &\le \min_{y_i\btheta^\sT\bd_i \ge \kappa}\left( \frac{\sfK}{2\kappa} + 1\right) \norm{\btheta}_2^2  \\
 &= \left( \frac{\sfK}{2\kappa} + 1\right)\widehat H_1^\bD(0,\kappa)\\
 &\stackrel{(b)}{\le}  2\left( \frac{\sfK}{2\kappa} + 1\right)\left(\frac{\kappa}{\kappa^\star}\right)^2
\end{align}
where $(a)$ follows by the domain of $s$: $|s| \oslambda \le 1/2$, and
 $(b)$ holds with high probability since $\widehat H_1^\bD(0,\kappa) \stackrel{\P}{\to} (\kappa/\kappa^\star)^2$.

For the norm of the minimizer note that
\begin{align}
2\left( \frac{\sfK}{2\kappa} + 1\right)\left(\frac{\kappa}{\kappa^\star}\right)^2
&\ge  \left(\norm{\widehat\btheta}_2 - |s|\norm{\Sigma}_\op \norm{\btheta^\star}_2\right) \norm{\widehat\btheta}_2\\
&\stackrel{(a)}\ge \left(\frac{\kappa}{\sfK} - |s|\oslambda \right)\norm{\widehat\btheta}_2\\
&\ge \frac{\kappa}{2\sfK} \norm{\widehat\btheta}_2,
\end{align}
where $(a)$ follows form the domain restriction on $s$.
Hence,
\begin{equation}
 \norm{\widehat\btheta}_2 \le 4 \frac{\sfK}{\kappa} \left( \frac{\sfK}{2\kappa} + 1\right)\left(\frac{\kappa}{\kappa^\star}\right)^2
\end{equation}
giving the desired statement for $l=1$.
Since the objective of $\widehat H_2^\bD(s,\kappa)$ is $|\btheta^\sT(\bI + s \bSigma) \btheta|$, the domain of $s$ along with the bound on $\widehat H_2(0,\kappa) = \widehat H_1(0,\kappa)$ above
directly imply the claim for $l=2$.
\end{proof}



\begin{lemma}
Fix $(s,L,l)  \in\sPi$. There exists $C(\kappa^\star) >0$ depending only on $\kappa^\star$ and $\oslambda$ such that for any $\epsilon\in(0,1)$, the following holds
with high probability on $\cG$:
 \begin{align}
 \widehat H_l^\bD(s,\kappa^\star + \epsilon) - C\epsilon  &\le \widehat H^\bD_l(s,\kappa^\star)  \le
 \widehat H_l^\bD(s,\kappa^\star - \epsilon)  + C \epsilon.
 \end{align}
\end{lemma}
\begin{proof}
 For $l=2$, these are immediate since we have
 \begin{align}
  \widehat H_2^\bD(s,\kappa^\star + \epsilon) &= 
 (1+\frac\epsilon{\kappa^\star})^2 \widehat H_2^\bD(s,\kappa^\star) \le  \widehat H_l^\bD(s,\kappa^\star) + 3\epsilon C_0(\kappa^\star) \\
  \widehat H_l^\bD(s,\kappa^\star - \epsilon) &= 
 (1-\frac\epsilon{\kappa^\star})^2 \widehat H_l^\bD(s,\kappa^\star) \ge  \widehat H_l^\bD(s,\kappa^\star) - 2\epsilon C_0(\kappa^\star) \\ 
 \end{align}
 where we used that $\widehat H_l^\bD \le C_0$ w.h.p. by the previous lemma.
 Meanwhile, for $l=1$, to show the first bound we write
 \begin{align}
  \widehat H^\bD_1(s,\kappa^\star + \epsilon) 
  %&= \min_{y_i\btheta^\sT\bg_i \ge \kappa(1+\epsilon)} \norm{\btheta}_2^2 + s C_1(\btheta)\\ 
  &= \min_{y_i\btheta^\sT\bg_i \ge \kappa} (1+\frac\epsilon{\kappa^\star})^2\norm{\btheta}_2^2 + (1+\frac\epsilon{\kappa^\star}) s C_1(\btheta)\\
  & \le \norm{\widehat\btheta}_2^2 (1+\frac\epsilon{\kappa^\star})^2 + s C_1(\widehat\btheta)(1+\frac\epsilon{\kappa^\star})\\
  &= (1+\frac\epsilon{\kappa^\star}) \widehat H_1^\bD(s,\kappa^\star)
   + \norm{\widehat\btheta}_2^2 \frac\epsilon{\kappa^\star}(1+\frac\epsilon{\kappa^\star})\\
   &\le \widehat H_1^\bD(s,\kappa^\star) + \frac\epsilon{\kappa^\star}\left(
   C_0 + C_1(\kappa^\star) (1+\frac\epsilon{\kappa^\star})
   \right)\\
   &\le \widehat H_1^\bD(s,\kappa^\star) + \epsilon C_2(\kappa^\star)
 \end{align}
 w.h.p.,
 where we used $\widehat\btheta :=\argmin_{y_i\bx_i^\sT\btheta \ge \kappa^\star}{\norm{\btheta}_2^2 + sC_1(\btheta)}$, and the previous lemma again.
 Similarly, the second bound is derived as
 \begin{align}
  \widehat H^\bD_1(s,\kappa^\star - \epsilon) 
  &= \norm{\widehat\btheta_\epsilon}_2^2 (1-\frac\epsilon{\kappa^\star})^2 + s C_1(\widehat\btheta_\epsilon)(1-\frac\epsilon{\kappa^\star})\\
  &= \norm{\widehat\btheta_\epsilon}_2^2 (1-\frac\epsilon{\kappa^\star}) + s C_1(\widehat\btheta_\epsilon)(1-\frac\epsilon{\kappa^\star})
     - \frac\epsilon{\kappa^\star} \norm{\widehat\btheta_\epsilon}_2^2\left(1-\frac\epsilon{\kappa^\star} \right)\\
     &\ge (1-\frac\epsilon{\kappa^\star}) \widehat H_1^\bD(s,\kappa^\star) 
     - \frac\epsilon{\kappa^\star} \norm{\widehat\btheta_\epsilon}_2^2\left(1-\frac\epsilon{\kappa^\star} \right)\\
     &= \widehat H_1^\bD(s,\kappa^\star)  - \frac\epsilon{\kappa^\star}\left( \widehat H_1^\bD(s,\kappa^\star)+ \norm{\widehat\btheta_\epsilon}_2^2\left(1-\frac\epsilon{\kappa^\star} \right) \right)\\
     &\ge \widehat H_1^\bD(s,\kappa^\star)  - \frac\epsilon{\kappa^\star} C_3(\kappa^\star)
 \end{align}
where $\widehat\btheta_\epsilon$ is the minimizer and we similarly used
the above lemma with $\kappa = \kappa^\star - \epsilon$.
\end{proof}



%\begin{lemma}
%Fix $(s,\kappa,L,l)  \in\sPi$. There exists $C >0$  such that for any $\epsilon\in(0,1)$, the following holds
%with high probability on $\cG$:
% \begin{align}
% \widehat H_l^\bD(s,\kappa(1+\epsilon)) - C\epsilon  &\le \widehat H^\bD_l(s,\kappa)  \le
% \widehat H_l^\bD(s,\kappa(1-\epsilon))  + C \epsilon.
% \end{align}
%\end{lemma}
%\begin{proof}
% For $l=2$, these are immediate since we have
% \begin{align}
%  \widehat H_2^\bD(s,\kappa(1+\epsilon)) &= 
% (1+\epsilon)^2 \widehat H_2^\bD(s,\kappa) \le  \widehat H_l^\bD(s,\kappa) + 3\epsilon C_0 \\
%  \widehat H_l^\bD(s,\kappa(1-\epsilon)) &= 
% (1-\epsilon)^2 \widehat H_l^\bD(s,\kappa) \ge  \widehat H_l^\bD(s,\kappa) - 2\epsilon C_0 \\ 
% \end{align}
% where we used that $\widehat H_l^\bD \le C_0$ w.h.p. by the previous lemma.
% Meanwhile, for $l=1$, to show the first bound we write
% \begin{align}
%  \widehat H^\bD_1(s,\kappa(1+\epsilon)) 
%  %&= \min_{y_i\btheta^\sT\bg_i \ge \kappa(1+\epsilon)} \norm{\btheta}_2^2 + s C_1(\btheta)\\ 
%  &= \min_{y_i\btheta^\sT\bg_i \ge \kappa} (1+\epsilon)^2\norm{\btheta}_2^2 + (1+\epsilon) s C_1(\btheta)\\
%  & \le \norm{\widehat\btheta}_2^2 (1+\epsilon)^2 + s C_1(\widehat\btheta)(1+\epsilon)\\
%  &= (1+\epsilon) \widehat H_1^\bD(s,\kappa)
%   + \norm{\widehat\btheta}_2^2 \epsilon(1+\epsilon)\\
%   &\le \widehat H_1^\bD(s,\kappa) + \epsilon\left(
%   C_0 + \norm{\widehat\btheta}_2^2 (1+\epsilon)
%   \right)\\
%   &\le \widehat H_1^\bD(s,\kappa) + \epsilon \widetilde C
% \end{align}
% where we used $\widehat\btheta :=\argmin_{y_i\bx_i^\sT\btheta \ge \kappa}{\norm{\btheta}_2^2 + sC_1(\btheta)}$, and that 
% $\widehat H_1^\bD(s,\kappa) + \norm{\widehat\btheta}_2^2 (1+\epsilon) \le \widetilde C$ on some high probability set (\notate{need to show this}).
% Similarly, the second bound is derived as
% \begin{align}
%  \widehat H^\bD_1(s,\kappa(1-\epsilon)) 
%  &= \norm{\widehat\btheta_\epsilon}_2^2 (1-\epsilon)^2 + s C_1(\widehat\btheta_\epsilon)(1-\epsilon)\\
%  &= \norm{\widehat\btheta_\epsilon}_2^2 (1-\epsilon) + s C_1(\widehat\btheta_\epsilon)(1-\epsilon)
%     - \epsilon \norm{\widehat\btheta_\epsilon}_2^2\left(1-\epsilon \right)\\
%     &\ge (1-\epsilon) \widehat H_1^\bD(s,\kappa) 
%     - \epsilon \norm{\widehat\btheta_\epsilon}_2^2\left(1-\epsilon \right)\\
%     &= \widehat H_1^\bD(s,\kappa)  - \epsilon\left( \widehat H_1^\bD(s,\kappa)+ \norm{\widehat\btheta_\epsilon}_2^2\left(1-\epsilon \right) \right)\\
%     &\ge \widehat H_1^\bD(s,\kappa)  - \epsilon \widetilde C
% \end{align}
%where $\widehat\btheta_\epsilon := \argmin_{y_i \bx_i^\sT\btheta \ge \kappa}\norm{\btheta}_2^2(1-\epsilon)^2 + s C_1(\btheta)(1-\epsilon)$ and we similarly used
%$\widehat H_1^\bD(s,\kappa)+ \norm{\widehat\btheta_\epsilon}_2^2\left(1-\epsilon \right) \le \widetilde C$ w.h.p.
%\notate{show this}.
%
%Now for a given $\delta$, take $\epsilon = \delta/\widetilde C$ to conclude 
%\begin{align}
% \lim_{n\to\infty} \P\left(\widehat H_l^\bX(s,\kappa) > L \right) &\le 
%  \lim_{n\to\infty} \P\left(\widehat H_l^\bD(s,\kappa(1+\epsilon)) > L  \right) \\
%  &\le \lim_{n\to\infty}
%  \P\left(\widehat H_l^\bD(s,\kappa) > L - \epsilon \widetilde C\right)
%\end{align}
%and
%\begin{align}
% \lim_{n\to\infty} \P\left(\widehat H_l^\bD(s,\kappa) \le L \right) &\le 
%  \lim_{n\to\infty} \P\left(\widehat H_l^\bD(s,\kappa(1-\epsilon)) \le L  \right) \\
%  &\le \lim_{n\to\infty}
%  \P\left(\widehat H_l^\bD(s,\kappa) \le L + \epsilon \widetilde C\right).
%\end{align}
%\end{proof}
%



==> simple-lemma-proof_bak.tex <==
%\newcommand{\op}{{\rm op}}

\newpage
\newcommand{\smin}{\sigma_{\rm min}}
\newcommand{\lmin}{\lambda_{\rm min}}
\newcommand{\lmax}{\lambda_{\rm max}}
\section{Proof of Lemma~\ref{lemma:restricted-strong-convexity}: Restricted Strong Convexity} 
\label{sec:proof-of-lemma-restricted-strong-convexity}

For $\bv=(v_i)_{i\leq p} \in \R^p$ and $\eps \in [0, \infty]$, define
$
    \norm{\bv}_{2,\eps}\equiv \max_{\btheta:\norm{\btheta}_2\leq 1\,,\, \norm{\btheta}_{\infty}\leq \eps}\big\langle \btheta,\bv\big\rangle\,.
$


Note, $\norm{\cdot}_{2,\eps}$ defines a norm. Moreover, 
$\eps \mapsto  \norm{\bv}_{2,\eps}$ is increasing for every $\bv$, and 
$\norm{\bv}_{2,\infty} = \norm{\bv}_2$.


The following result generalizes Lemma~\ref{lemma:restricted-strong-convexity}.
\begin{lemma}
\label{lemma:RSC_inf_norm}
Given any deterministic sequence $\{\eps_n\}_{n\geq 1}$ such that $\sqrt{n}\eps_n \to\infty$, there are 
constants $c, c_1, c_2 > 0$, and $N_0$ independent of $n$ such that for every $n \ge N_0$, the event
\begin{equation}
\label{eqn:proof-restricted-strong-convexity-eps}
	\norm{\bX \bu}_{2,\eps_n} \ge c_1\sqrt{n} \norm{\bu}_2 - c_2 \norm{\bu}_1~~\text{for all $\bu \in \R^n$}
\end{equation} 
holds with probability at least $1- o_n(1)$. 
\end{lemma}

\subsection{The Main Argument} 
\label{sec:main-geometric-argument}
%that can only depend on $\gamma$. 
We define a ``good'' event $\Omega$ which is the intersection of two subevents $\Omega_1, \Omega_2$: 
\begin{itemize}
\item $\Omega_1$: the matrix $\bX$ has its operator norm bounded by $\norm{\bX}_\op \le c_0\sqrt{n}$ 
(section~\ref{sec:bound-on-operator-norm}).
\item $\Omega_2$: for every submatrix $\bX_S$, where $S$ has its cardinality equal to 
$c_3 n$ and $\bX_S$ denotes $p\times|S|$ matrix with columns $(\bX_i)_{i\in S}$, we have
	$\norm{\bX_S\bu_S}_{2,\eps_n} \ge c_4\sqrt{n}\norm{\bu_S}_2$ (see Section~\ref{sec:bound-on-restricted-eigenvalue}).
\end{itemize}
Lemma~\ref{lemma:operator-norm-bound-on-Z} and~\ref{lemma:restricted-minimum-singular-value} 
show, if $c_0, c_3, c_4$ are chosen appropriately, then the event 
$\Omega=\Omega_1\cap \Omega_2$ happens with probability at least $1- o_n(1)$. Here, 
$c_0, c_3, c_4$ are constants which do not depend on $n$. 

Given $\Omega$, below we prove the bound~\eqref{eqn:proof-restricted-strong-convexity-eps} always 
holds on the event $\Omega$ with $c_1 = c_4 \sqrt{c_3}$, and $c_2 = c_0/\sqrt{c_3}$.

Our proof is based on a series of elementary inequalities. 
Let $\Omega$ happen. Fix $\bu \in \R^n$. Order its coordinates as
\begin{equation*}
	|\bu_{i_1}| \ge |\bu_{i_2}| \ge \ldots |\bu_{i_n}|.
\end{equation*}
Let $S = \{i_1, i_2, \ldots, i_k\}$ where $k = c_3 n$. Note $\bX \bu = \bX_S \bu_S + \bX_{S^c} \bu_{S^c}$. 
By triangle inequality, there is 
\begin{equation}
\label{eqn:initial-triangle-inequality}
\begin{split}
	\norm{\bX \bu}_{2,\eps_n}  &\ge \norm{\bX_S \bu_S}_{2,\eps_n} - \norm{\bX_{S^c} \bu_{S^c}}_{2,\eps_n} \\
		&\ge c_4 \sqrt{n}\norm{\bu_{S}}_2 - c_0 \sqrt{n}\norm{\bu_{S^c}}_2.
\end{split} 
\end{equation} 
where the second inequality follows from the definition of $\Omega_1, \Omega_2$, and the fact that 
$\norm{\bv}_{2, \eps} \le \norm{\bv}$.

Here are some basic estimates of $\norm{\bu_{S}}_2$ and $\norm{\bu_{S^c}}_2$.
Since $\bu_S$ contains coordinates with largest absolute entries, 
\begin{equation*}
	\norm{\bu_S}_2 \ge \sqrt{|S|/n} \norm{\bu}_2 = \sqrt{c_3} \norm{\bu}_2.
\end{equation*} 
Similarly, since $\bu_{S^c}$ contains coordinates with smallest absolute entries,
\begin{equation*}
	\norm{\bu_{S^c}}_2  \le \norm{\bu_{S^c}}_1^{1/2} \norm{\bu_{S^c}}_\infty^{1/2}
		\le \norm{\bu_{S^c}}_1^{1/2} \cdot (\norm{\bu_S}_1/|S|)^{1/2} = \norm{\bu}_1/\sqrt{c_3 n}.
\end{equation*} 
Substitute the above estimates 
into equation~\eqref{eqn:initial-triangle-inequality}, we obtain 
$
	\norm{\bX \bu}_{2,\eps_n} \ge c_4 \sqrt{c_3 n}\norm{\bu}_2 - c_0/\sqrt{c_3} \norm{\bu}_1. 
$
As the bound holds for all $\bu$, this completes the proof. 

\newcommand{\Q}{\mathbf{Q}}
\subsection{Subgaussianity Properties of Rows}

\subsubsection{Random Feature Ensemble} 

Recall the random feature ensemble $\bX = \sigma (\bW \bZ) \in \R^{p \times n}$ where 
$\bW \in \R^{p \times d}$ has i.i.d. entries $\normal(0, 1/d)$ and 
$\bZ \in \R^{d \times n}$ has i.i.d. entries $\normal(0, 1)$. 

We recall the definition of subgaussianity. 
\begin{definition}
A probability distribution $\Q$ on $\R^p$ is called subgaussian with parameter $\nu^2$ if 
it has mean $\E_{Q}[\bq] = 0$ and 
\begin{equation*}
	\text{$\E_{Q}[e^{\langle \bq, \bu\rangle}] \le e^{\nu^2 \norm{\bu}_2^2/2}$ holds for all vectors $u \in \R^p$. }
\end{equation*} 
\end{definition}

%Let $\sigma(\bZ)$ denote the sigma-field generated by matrix $\bZ$. 
Lemma~\ref{lemma:crazy-lemma-random-feature-models} shows that the random matrix 
ensemble $\bX$ has independent subgaussian rows when conditional on $\bZ$. Additionally,
after this conditioning, the subgaussianity parameter as well as the minimum  and maximum 
eigenvalue of the covariance of the row of $\bX$ are properly behaved with high probability. 

For clarity, Lemma~\ref{lemma:crazy-lemma-random-feature-models} is stated in a nonasymptotic setting
where the size of the matrix $n, p, d$ are fixed. 

\begin{lemma}[Property of Random Feature Ensemble]
\label{lemma:crazy-lemma-random-feature-models}
There are universal constants $c, C$ such that the following holds. 
For every $n, p, d$, the event $\Omega_{\bZ}$ of the following form: 
	\begin{equation*}
		\Omega_{\bZ} = \left\{\norm{\bZ}_\op \le C(\sqrt{d}+\sqrt{p}),~~\max_i \norm{\bz_i}_2 \le C\sqrt{\log n}, 
			~~\max_{i, j\le n, i \neq j}|\langle \bz_i, \bz_j\rangle| \le C\log n\right\}
	\end{equation*}
satisfies the following three properties:  
\begin{itemize}
\item $\Omega_{\bZ}$ happens with probability at least $1-n^{-1} - e^{-cp}$. 	
\item Conditional on $\bZ$, the rows of $\bX$ are i.i.d.
	subgaussian with parameter $\nu^2(\bZ)$. Furthemore, on the event $\Omega_{\bZ}$,
	\begin{equation*}
		\nu(\bZ) \le C (1+\sqrt{p/d}) \norm{\sigma}_{{\rm lip}}.
	\end{equation*} 
\item Let $\bSigma_{\bZ}$ denote the conditional covariance $\bX$ given $\bZ$, where $\bX$ stands for a row of $\bX$.
	Then on the event $\Omega_{\bZ}$,
	\begin{equation*}
		\mu_2 - \delta_n 
			\le \lambda_{\min}(\bSigma_{\bZ}) \le \lambda_{\max}(\bSigma_{\bZ}) \le C\mu_1 \cdot (1+\sqrt{p/d}) + \mu_2 
			+ \delta_n
	\end{equation*}
	where $|\delta_n| \le \frac{C}{\sqrt{n}}((1+\sqrt{p/d})^4 + \log^4 n)$. 
\end{itemize}
\end{lemma}

The proof of Lemma~\ref{lemma:crazy-lemma-random-feature-models} is deferred to 
Section~\ref{sec:proof-crazy-lemma-random-feature-models}.  

\subsubsection{Independent Feature Ensemble} 
The random matrix ensemble $\bX$ has independent rows, which is subgaussian with 
parameter at most $\nu^2$. Each row has covariance 
whose eigenvalue is lower bounded by $\lambda_{\min}(\bSigma_{{\sf ind}})$.



\subsection{Event  $\Omega_1$}
\label{sec:bound-on-operator-norm}
This section proves Lemma~\ref{lemma:operator-norm-bound-on-Z} which says, 
with appropriate $c_0$, the event $\Omega_1$ (see Section~\ref{sec:main-geometric-argument}
for a definition of this event) happens with high probability. 

\begin{lemma}[Operator Norm]
\label{lemma:operator-norm-bound-on-Z}
Let $p/d= \kappa$. For some universal constant $c > 0$, and constant $c_0 > 0$ depending only on 
$\kappa, \norm{\sigma}_{{\rm lip}}, \mu_1, \mu_2$, with probability at least $1-e^{-cp}$ the matrix $\bX$ 
satisfies
\begin{equation*}
	\norm{\bX}_\op \le c_0 (\sqrt{n} + \sqrt{p}).
\end{equation*}
\end{lemma}



%\notate{I will split the proof of Lemma 19 soon.}






\newcommand{\lip}{{\rm lip}}


\begin{proof}
The proof is divided into two cases, depending on what $\bX$ refers to. 

\paragraph{Random Feature Ensemble} 
Let $\Omega_Z$ denote the event for which Lemma~\ref{lemma:crazy-lemma-random-feature-models} holds. 

By Theorem~\ref{theorem:matrix-concentration-covariance-operator} and 
Lemma~\ref{lemma:operator-norm-bound-on-Z}, there are universal constants $c, C > 0$ such that
\begin{equation*}\label{eq:approx:D}
    \bigg\|\frac{1}{p}\bX^{T}\bX-\bSigma_{\bZ}\bigg\|_{\op}\leq  C \nu^2(\bZ)
    	\bigg(\sqrt{\frac{n}{p} + 1}+ \frac{n}{p} + 1\bigg)~~\text{holds with probability at least $1-e^{-c p}$}, 
\end{equation*} 
where there's further the high probability bound 
\begin{equation*}
	\nu(\bZ) \le C \left(1+\sqrt{\kappa}\right) \norm{\sigma}_{{\rm lip}}~~\text{and}~~
	 \lambda_{\max}(\bSigma_{\bZ}) \le C \mu_1 \left(1+\sqrt{\kappa}\right) + \mu_2 
			+ \delta_n
\end{equation*}
for some $\delta_n \le \frac{C}{\sqrt{n}} ((1+\sqrt{\kappa})^4 + \log^4 n)$ which tends to $0$ as $n \to \infty$. 
This result implies Lemma \ref{lemma:operator-norm-bound-on-Z}.
 
\paragraph{Independent Feature Ensemble}  
$\bX$ has independent rows with subgaussianity parameter $\nu^2$ where $\nu < \infty$.

Lemma \ref{lemma:operator-norm-bound-on-Z} then
follows immediately  from Theorem~\ref{theorem:matrix-concentration-covariance-operator}.
 
\end{proof} 
%\end{enumerate}


\subsection{Event $\Omega_2$} 
\label{sec:bound-on-restricted-eigenvalue}
Lemma~\ref{lemma:restricted-minimum-singular-value} says with appropriate $c_3, c_4$, the event $\Omega_2$  (see Section~\ref{sec:main-geometric-argument}
for the defintion) happens with high probability. 

\newcommand{\norms}[1]{\|#1\|}

\begin{lemma}%[Restricted Minimum Singular Value]
\label{lemma:restricted-minimum-singular-value}
Given any $\eps_n>0$ with $\sqrt{n}\eps_n\to\infty$ as $n\to\infty$, there are constants $c_3, c_4 > 0$
depending only on $\sgamma_1, \sgamma_2, \mu_1, \mu_2$, such that the event
\begin{equation*}
	\min_{\bv:\norm{\bu}_2=1}\norm{\bX_{S}\bu}_{2,\eps_n}\geq c_4 \sqrt{n}~~\text{for every subset 
		$S \subseteq [n]$, $|S| = c_3 n$}
\end{equation*} 
holds with probability tending to one as $n \to \infty$.
\end{lemma}

Our proof is based on two general statements. The first is a lower bound on $\norm{\cdot}_{2, \eps}$, 
see Section~\ref{sec:lower-bound-norm-two-eps}. The second is a generalization of Kashin's 
theorem, providing sufficient conditions on a random matrix $\bA$ with independent rows such that
with high probability $\norm{\bv}_1 \approx \frac{1}{\sqrt{p}} \norm{\bv}_2$ holds uniformly over 
$\bv$ in the column space of $\bA_S$ for proper size $S$, see 
Section~\ref{sec:equivalence-between-ell-one-ell-two-random-subspaces}. 




\subsubsection{Lower Bound on Norm $\norm{\cdot}_{2, \eps}$}
\label{sec:lower-bound-norm-two-eps}
\begin{lemma}
\label{lemma:elementary}
For every $\bv \in \R^p, \eps > 0$, there is 
$\norm{\bv}_{2, \eps} \ge \norm{\bv}_2 \cdot \left(\frac{\norm{\bv}_1}{\sqrt{p}\norm{\bv}_2} - \frac{1}{\sqrt{p}\eps}\right)_+^2$.
\end{lemma}
\begin{proof}
Write $\bv=(v_i)_{i\leq p} \in \R^p$.  Since every norm is homogeneous, 
it suffices to prove the lemma when $\norm{\bv}_2 = 1$.

Let $T(\eps) = \{i: |v_i| \le \eps\}$. Then $\norm{\bv}_{2, \eps}  \ge  \norms{\bv_{T(\eps)}}_2^2$.
Indeed, $\norm{\bv}_{2, \eps} \ge \langle\bv, \btheta \rangle$ where $\btheta_i= v_i$
for $i \in T(\eps)$ and $\btheta_i = 0$ for $i \in T^c(\eps)$.
Note $ \norms{\bv_{T(\eps)}}_2 \ge \frac{1}{\sqrt{p}}  \norms{\bv_{T(\eps)}}_1$ where
$\norms{\bv_{T(\eps)}}_1 = \norm{\bv}_1 - \norms{\bv_{T^c(\eps)}}_1$ by Cauchy-Schwartz. The result follows 
since $\norms{\bv_{T^c(\eps)}}_1 \le \norms{\bv_{T^c(\eps)}}_2^2/\eps$ by Markov's inequality, and
$\norms{\bv_{T^c(\eps)}}_2\le \norm{\bv}_2 = 1$. 
\end{proof}

\subsubsection{Equivalence between $\ell_1$ and $\ell_2$ norm in Random Subspaces} 
\label{sec:equivalence-between-ell-one-ell-two-random-subspaces}
Below is the main result of the Section. 
\begin{lemma}
\label{lemma:equivalence-between-l1-and-l2-norm}
Let $\bA\in \R^{p\times n}$ be a random matrix whose rows $\{\ba_i\}_{i\leq p}\in \R^n$ are i.i.d. subgaussian
with parameter $\nu^2$. Suppose, for some $\kappa > 0$, the covariance $\bSigma_J \equiv \E [\ba_J \ba_J^{T}]$ 
satisfies $\lmin(\bSigma_J)\ge \kappa \nu^2$ for every $J$ where
$|J| \ge N$. Then there's a constant $c' = c'(\kappa)$ depending
only on $\kappa$ such that 
for $m = c' p$, given any subset $S$ with $N \le |S| \le m$, 
\begin{equation}
\label{eqn:equivalence-between-l1-l2}
		 \frac{1}{\sqrt{p}}\norm{\bA_S u}_2 \ge \norm{\bA_S u}_1 \ge  \frac{c}{\sqrt{p}} \norm{\bA_S u}_2
		 	~~\text{for every $u \in \R^{|S|}$}
\end{equation}
holds with probability at least $1-e^{-cp}$. Here $c > 0$ is a universal constant. 
\end{lemma} 

The first inequality in equation~\eqref{eqn:equivalence-between-l1-l2} always holds by Cauchy-Schwartz inequality. 
The second inequality that holds uniformly over $u \in \R^{cn}$ is where random 
matrix theory comes in. 

Lemma~\ref{lemma:equivalence-between-l1-and-l2-norm} follows from two results: 
Lemma~\ref{lemma:lower-bound-on-l-1-norm} and
Lemma~\ref{lemma:upper-bound-on-l2-norm}.

\begin{lemma}
\label{lemma:lower-bound-on-l-1-norm}
Let $\bA\in \R^{p\times m}$ be a random matrix whose rows $\{\ba_i\}_{i\leq p}\in \R^m$ are i.i.d. subgaussian
with parameter $\nu^2$. Suppose the covariance $\bSigma\equiv \E [\ba \ba^{T}]$ satisfies 
$\lmin(\bSigma)\ge \kappa \nu^2$ where $\kappa > 0$. Then, there are constants $C_1, C_2 > 0$ depending only on 
$\kappa$, and a universal constant $c > 0$, such that with probability at least $1-e^{-cp}$, 
\begin{equation}
%\frac{1}{\sqrt{p}}\norm{\bA \bv}_{1}\geq  (C_1 - C_2 \sqrt{m/p})_+^2 \norm{\bA \bv}_2
	\norm{\bA \bv}_{1} \ge p \nu (C_1 - C_2 \sqrt{m/p})_+ \cdot \norm{\bv}_2~~\text{holds for every $\bv$}.
\end{equation}
\end{lemma}
\begin{proof}
Let $\sigma > 0$ be determined later. Note by Markov's inequality, for every vector $\bv$
\begin{equation*}
	\norm{\bA \bv}_{1}
		\ge \sigma \cdot \sum_{j} \mathbf{1}_{|\langle \ba_j, \bv\rangle|\ge \sigma}. 
\end{equation*}
A standard VC argument~\cite[Section 4]{Wainwright19} yields that, for some universal constant $C, c > 0$: 
\begin{equation*}
	\sup_{\bv} |\frac{1}{p}\sum_{j} \mathbf{1}_{|\langle \ba_j, \bv\rangle|\ge \sigma}
		- \P(|\langle \ba, \bv\rangle| \ge \sigma)| \le C \sqrt{m/p}
\end{equation*}
with probability at least $1- e^{-cp}$. So with triangle inequality, this implies with at least 
the same probability we have 
\begin{equation*}
	 \norm{\bA \bv}_{1} \ge 
		p\sigma \cdot (\min_{\bv: \norm{\bv}_2 = 1} \P(|\langle \ba, \bv\rangle| \ge \sigma) - C \sqrt{m/p})_+ 
			\cdot \norm{\bv}_2~~\text{for every $\bv$}.
\end{equation*} 
Below we lower bound $\P(|\langle \ba, \bv\rangle| \ge \sigma)|$ for every $\sigma > 0$ and $\bv$ with 
$\norm{\bv}_2 = 1$. 

Write $z = \langle \ba, \bv \rangle$ where  $\norm{\bv}_2 = 1$. Note $\E[z^2] \ge  \kappa \nu^2$, and 
$\E[z^4] \le C\nu^4$ for a universal constant $C < \infty$.  Hence, 
$\E[z^2 \mathbf{1}_{|z| \ge \sigma}] \le \frac{C \nu^4}{\sigma^2}$ by Markov's inequality,
which yields $\E[z^2\mathbf{1}_{|z| \le \sigma}] \ge \kappa \nu^2- \frac{C \nu^4}{\sigma^2}$. 
Hence $\P(|z| \le \sigma) \ge \frac{\kappa \nu^2}{\sigma^2} - \frac{C \nu^4}{\sigma^4}$. 
As a result, this means there are $C_1, C_2 > 0$ depending only on $\kappa$ such that 
$\P(|\langle \ba, \bv\rangle| \ge C_1 \nu) \ge C_2$ .

This proves that with probability at least $1- e^{-cp}$,
\begin{equation*}
\text{$\norm{\bA \bv}_{1} \ge C_1 p \nu (C_2 - C \sqrt{m/p})_+ \cdot \norm{\bv}_2$ holds for every 
$\bv$.}
\end{equation*}


%By Theorem xxx, there's also the other event that holds with probability at least $1-e^{-c' p}$: 
%\begin{equation*}
%	\norm{\bA \bv}_{2} \le C' \sqrt{p} \nu (1 + \sqrt{m/p}) \cdot \norm{\bv}_2~~\text{for every $\bv$}.
%\end{equation*} 
%where both constants $c', C'$ are absolute constants. The desired Lemma
\end{proof}


\begin{lemma}
\label{lemma:upper-bound-on-l2-norm}
Let $\bA\in \R^{p\times m}$ be a random matrix whose rows $\{\ba_i\}_{i\leq p}\in \R^m$ are i.i.d. subgaussian
with parameter $\nu^2$. Then, there are universal constants $c, C > 0$ such that with probability at least $1-e^{-cp}$
\begin{equation*}
	\norm{\bA \bv}_2 \le C \sqrt{p} \nu ( 1+ \sqrt{m/p}) \cdot \norm{\bv}_2~~\text{holds for every $\bv$}. 
\end{equation*}
\end{lemma}
\begin{proof}
This follows from results in 
nonasymptotic random matrix theory (Theorem~\ref{theorem:matrix-concentration-covariance-operator}).
\end{proof} 



\subsubsection{Proof of Lemma~\ref{lemma:restricted-minimum-singular-value}}
Here's the main idea of the proof. 
By Lemma~\ref{lemma:elementary}, we know 
\begin{equation}
\label{eqn:initial-lower-bound}
	\norm{\bX_S \bu}_{2, \eps_n} \ge \norm{\bX_S \bu}_2 \cdot \left(\frac{\norm{\bX_S \bu}_1}
		{\sqrt{p}\norm{\bX_S \bu}_2} - \frac{1}{\sqrt{p} \eps_n}\right)_+^2
\end{equation}
We shall lower bound the RHS by $c_4 \sqrt{p}$, 
uniformly over all indices $S$ with cardinality $c_3 n$, and vector $u \in R^{|S|}$, with 
probability tending to one.
Here $c_3, c_4 > 0$ are constants to be determined in the rest of the proof. 

For the remainder, we divide our proof into two cases, depending on the random matrix 
ensemble $\bX$. 

Let $\kappa = p/d, \kappa'=n/p$. 

\paragraph{Random Feature Ensemble} 
$\bX$ is the random feature ensemble. 

By Lemma~\ref{lemma:crazy-lemma-random-feature-models}, we can choose a proper event 
	\begin{equation*}
		\Omega_{\bZ} = \left\{\norm{\bZ}_\op \le C(\sqrt{d}+\sqrt{p}),~~\max_i \norm{\bz_i}_2 \le C\sqrt{\log n}, 
			~~\max_{i, j\le n, i \neq j}|\langle \bz_i, \bz_j\rangle| \le C\log n\right\}
	\end{equation*}
which happens with probability at least $1-n^{-1} - e^{-cp}$, where $c, C > 0$ are universal constants, such that 
the following holds. 
There exists an $N_0$ such that for every index $S$ such that $|S| \ge N_0$, we have 
\begin{itemize}	
\item Conditional on $\bZ$, the rows of $\bX_S$ are i.i.d.
	subgaussian with parameter $\nu^2(\bZ)$. Furthemore, on the event $\Omega_{\bZ}$,
	\begin{equation*}
		\nu(\bZ) \le C (1+\sqrt{\kappa}) \norm{\sigma}_{{\rm lip}}.
	\end{equation*} 
\item Let $\bSigma_{\bZ, S}$ denote the conditional covariance $\bX_S$ given $\bZ$, where $\bX$ stands for a row of $\bX$.
	Then on the event $\Omega_{\bZ}$,
	\begin{equation*}
		\frac{1}{2} \mu_2 
			\le \lambda_{\min}(\bSigma_{\bZ, S}) \le \lambda_{\max}(\bSigma_{\bZ, S}) \le C\mu_1 \cdot (1+\sqrt{\kappa}) + 2\mu_2. 
	\end{equation*}
\end{itemize}

By Lemma~\ref{lemma:equivalence-between-l1-and-l2-norm} and
Theorem~\ref{theorem:matrix-concentration-covariance-operator}, 
there is a constant $c_3$ depending only on 
$\mu_1, \mu_2, \kappa, \kappa'$ such that the following two bounds hold 
for every given individual subset $S$ where $N_0 \le |S| \le c_3 n$ on the event $\Omega_{\bZ}$.
The first is the bound below holds with probability at least $1-e^{-cp}$ for some universal constant $c > 0$: 
\begin{equation}
\label{eqn:key-bound-high-probability-one}	
	\inf_{\bu: \bu \in \R^{|S|}} \frac{\norm{\bX_S \bu}_1}{\sqrt{p}\norm{\bX_S \bu}_2} \ge c_3,
\end{equation}
and the second is the bound below holds with probability at least $1-e^{-cp}$ for some $c > 0$
depending only on $\mu_2$: 
\begin{equation}
\label{eqn:key-bound-high-probability-two}
	\inf_{\bu: \bu \in \R^{|S|}, \norm{\bu}_2 = 1} \norm{\bX_S \bu}_2 \ge \frac{\mu_2}{4}\sqrt{p}. 
\end{equation} 

We make these lower bounds uniform over $|S| = c_3 n$ when $c_3$ is sufficiently small. Note the 
number of sets $S$ with cardinality $|S| = c_3 n$ is bounded by $\exp(n H(c_3))$, where 
$H(x) = -x\log_2 (x) - (1-x) \log_2 (1-x)$ is the entropy. Note $H(c_3) \to 0$ as $c_3 \to 0$.
This means that we can take $c_3, c$ depending 
on $\mu_1, \mu_2, \kappa, \kappa'$ such that with probability at least $1-e^{-cp}$, 
the above bounds~\eqref{eqn:key-bound-high-probability-one}
and~\eqref{eqn:key-bound-high-probability-two} hold uniform over set $S$ with cardinality $|S| = c_3 n$
on the event $\Omega_{\bZ}$.

Finally, since $\sqrt{p} \eps_n \to 0$ as $n \to \infty$, we may assume $\frac{1}{\sqrt{p}\eps_n} \le \frac{c_3}{2}$
for $n \ge N_0$.

These uniform bounds, in conjunction with~\eqref{eqn:initial-lower-bound}, allow us to conclude that for every 
$n \ge N_0$, 
\begin{equation*}
	\inf_{S: |S| = c_3 n}\inf_{\bu: \bu \in \R^{|S|}, \norm{\bu}_2 = 1}\norm{\bX_S \bu}_{2, \eps_n} \ge c_4 \sqrt{p}
\end{equation*}
holds with probability at least $1-e^{-cp}$ on the event $\Omega_{\bZ}$. 
In the above, $c, c_3, c_4, N_0$ depend only on $\mu_1, \mu_2, \kappa, \kappa'$. The result now 
follows since $\Omega_{\bZ}$ holds with probability tending to one, as $n \to \infty$. 

\paragraph{Independent Feature Ensemble} 
$\bX$ is the independent feature ensemble. 

We start by noticing the very basic property of $\bX_S$ for every index subset $S$. 
Note the rows $\bX_S$ are independent and subgaussian with parameter at most $\nu^2$, 
with the eigenvalue of the covariance lower bounded by $\gamma > 0$. Here, $\nu, \gamma$
are constants independent of $n, d, p$.

By Lemma~\ref{lemma:equivalence-between-l1-and-l2-norm} and
Theorem~\ref{theorem:matrix-concentration-covariance-operator}, 
there are constants $c_3, c$ depending only on 
$\nu, \gamma, \kappa, \kappa'$ such that  
for every given individual subset $S$ where $|S| \le c_3 n$,
the following bounds hold with probability at least $1-e^{-cp}$. The first bound is 
\begin{equation}
\label{eqn:key-bound-high-probability-one-ind}	
	\inf_{\bu: \bu \in \R^{|S|}} \frac{\norm{\bX_S \bu}_1}{\sqrt{p}\norm{\bX_S \bu}_2} \ge c_3,
\end{equation}
and the second bound is: 
\begin{equation}
\label{eqn:key-bound-high-probability-two-ind}
	\inf_{\bu: \bu \in \R^{|S|}, \norm{\bu}_2 = 1} \norm{\bX_S \bu}_2 \ge \frac{\gamma}{2}\sqrt{p}. 
\end{equation} 
The remainder of the proof is very similar to that of the random feature ensemble. 

We make these lower bounds uniform over $|S| = c_3 n$ for sufficiently small $c_3$. This 
is doable, as the number of  sets $S$ with cardinality $|S| = c_3 n$ is bounded by $\exp(n H(c_3))$
where $H(c_3) \to 0$ as $c_3 \to 0$. Thus, we can say the above 
bounds~\eqref{eqn:key-bound-high-probability-one-ind}
and~\eqref{eqn:key-bound-high-probability-two-ind} hold uniform over set $S$ with probability 
tending to one. 

Finally, note $\sqrt{p} \eps_n \to 0$. This allows us to conclude that for some $c_3, c_4$: 
\begin{equation*}
	\inf_{S: |S| = c_3 n}\inf_{\bu: \bu \in \R^{|S|}, \norm{\bu}_2 = 1}\norm{\bX_S \bu}_{2, \eps_n} \ge c_4 \sqrt{p}
\end{equation*}
holds with probability tending to one as $n \to \infty$, where, $c_3, c_4$ depend only on 
$\gamma, \nu, \kappa, \kappa'$. The proof is thus complete. 

\subsection{Proof of Lemma~\ref{lemma:crazy-lemma-random-feature-models}}
\label{sec:proof-crazy-lemma-random-feature-models}
Throughout this proof, we conditional on $\bZ$. 

Clearly, the rows of $\bX$ are independent copies of $\bX = 
\sigma(\bZ^T \bw)$ where $\bw \sim \normal(0, I_d/d)$. Note 
$\bw \mapsto \langle \bv, \sigma(\bZ^T \bw)\rangle$ is Lipschitz with Lipschitz constant 
at most $\norm{\bZ}_\op \norm{\bv}_2 \norm{\sigma}_{{\rm lip}}$. Hence, 
$\bX$ is subgaussian with parameter 
\begin{equation}
	\nu(\bZ) = \frac{C}{\sqrt{d}} \cdot \norm{\bZ}_\op \norm{\sigma}_{{\rm lip}}.
\end{equation} 
for some universal 
constant $C > 0$. Furthermore, the covariance matrix of $\bX$, denoted by $\bSigma_{\bZ}$, is given by 
\begin{equation*}
	\bSigma_{\bZ} \equiv \Big(\bSigma_{\bZ}(k,\ell)\Big)_{k,\ell\leq n}\equiv \bigg(\E_{\bw} \Big[\sigma\big(\langle \bw, \bz_{k}\rangle\big)\cdot \sigma(\big\langle \bw, \bz_{\ell}\big\rangle)\Big]\bigg)_{k,\ell\leq n}\,,
\end{equation*} 
where $\bz_{1},\ldots,\bz_{n}$ are columns of $\bZ$ and $\E_{\bw}$ denotes the expectation with 
respect to $\bw$ conditioned on $\bZ$.

Let us denote $\bSigma_{\bZ}^\prime\equiv \frac{\mu_1^2}{d}\bZ^{T}\bZ + \mu_2^2 \bI_n$.
Introduce $\kappa_n =  \max_{1\le i, j \le n} \sqrt{d}\cdot |\frac{1}{d}\langle \bz_i, \bz_j\rangle - \mathbf{1}_{i = j}|$, 
and $\zeta_n = \norm{\bZ}_\op/\sqrt{d}$. According to \cite[Lemma 5]{HuLu22}, 
There is a constant $C > 0$ independent of $n$ such that with probability one there holds
\begin{equation*}
%\label{eqn:bound-for-kernels}
	\norm{\bSigma_{\bZ} - \bSigma_{\bZ}^\prime}_\op \le \delta_n(\bZ)
\end{equation*}
where $\delta_n(\bZ) = C \cdot \frac{ 1+ \kappa_n^3 + \zeta_n^4 }{\sqrt{n}}$. Hence, we may use 
triangle inequality to obtain the bound 
\begin{equation}
	\mu_2 - \delta_n(\bZ) \le \lambda_{\min}(\bSigma_{\bZ}) \le \lambda_{\max} (\bSigma_{\bZ}) \le 
		\mu_1 \cdot \frac{\norm{\bZ}_\op}{\sqrt{d}} + \mu_2 + \delta_n(\bZ).
\end{equation}

To finish the proof, we give bounds on $\nu^2(\bZ)$, as well as $\delta_n(\bZ)$ that holds with high probability. 

\begin{itemize}
\item 
By Theorem~\ref{theorem:matrix-concentration-covariance-operator}, $\norm{\bZ}_\op \le C (\sqrt{p} + \sqrt{d})$
with probability at least $1-e^{-cp}$. Here, $C, c$ are universal constants. 

\item 
By \cite[Theorem 3.1.1]{Vershynin18}, $|\norm{\bz}_2 - \sqrt{d}|$ is subgaussian with parameter 
$c$ where $c > 0$ is universal. A union bound then shows 
$\max_{i \le n} |\norm{\bz_i}_2 - \sqrt{d}| \le C \sqrt{\log n}$ holds 
with probability at least $1-\frac{1}{2n}$ for some universal constant $C$. Also, one can show that 
$\max_{i, j \le n, i\neq j} |\langle z_i, z_j\rangle| \le C \log n$ with probability at least $1-\frac{1}{2n}$
for some large universal constant $C > 0$. 

This shows that $|\delta_n(\bZ)| \le \frac{C}{\sqrt{n}}((1+\sqrt{p/d})^4 + \log^4 n)$ with probability at least $1-n^{-1}$. 
\end{itemize}

Now we simply define $\Omega_{\bZ}$ as the event for which the conclusions of the above two bullet points 
hold. Lemma~\ref{lemma:crazy-lemma-random-feature-models} then follows from the above discussions. 

\subsection{Random Matrix Theory Tools} 
The following result is a restatement of Theorem 6.5 from \cite{Wainwright19}.

\begin{theorem}[Matrix Concentration]
\label{theorem:matrix-concentration-covariance-operator}
Let $\bA \in \R^{p \times m}$ be a random matrix whose rows $\{\ba_i\}_{i\leq p}\in \R^m$ are i.i.d drawn from a 
subgaussian distribution with parameter $\nu^2 > 0$. Denote the covariance matrix by $\bSigma \equiv \E \ba_i\ba_i^{T}$. Then there exist absolute constants $c, C \in (0, \infty)$ such that for every $\delta > 0$
\begin{equation*}	
	\bigg\|\frac{1}{p}\bA^{T} \bA - \bSigma\bigg\|_\op \le 
		C\cdot \nu^2 \bigg(\sqrt{\frac{m}{p} + \delta}+ \frac{m}{p} + \delta\bigg)~~\text{holds with probability at least $1-e^{-c p \delta}$}.
\end{equation*}
\end{theorem}

%
%\newpage
%
%
%
%
%
%\begin{lemma}\label{lem:min:eval:deloc}
%Let $\eps_n>0$ satisfy $\eps_n\to 0$ and $\sqrt{n}\eps_n\to\infty$ as $n\to\infty$. Let $\bA\in \R^{p\times m}$ be a random matrix whose rows $\{\ba_i\}_{i\leq p}\in \R^m$ are i.i.d. drawn from a subgaussian distribution with parameter $\nu^2>0$. Suppose the covarinace matrix $\bSigma\equiv \E \ba_i \ba_i^{T}$ satisfy $\lambda_{\sf m}\leq \lmin(\bSigma)\leq \lmax(\bSigma)\leq \lambda_{\sf M}$ for some constants $\lambda_{\sf m}, \lambda_{\sf M}>0$. Then, there exists a constant $C_1, C_2, C_3$, which only depends on $\nu, \lambda_{\sf m}, \lambda_{\sf M}>0$ such that the following holds. If $m\leq C_1 p$, then with probability at least $1-e^{-C_2 p}$, we have
%\begin{equation*}	
%	\min_{\bv: \norm{\bv}_2=1}\norm{\bA \bv}_{2,\eps_n}\geq C_3 \sqrt{p} ~~~\text{holds with probability at least $1-e^{-C_2 p}$}.
%\end{equation*}
%\end{lemma}
%\begin{proof}
%Throughout, we let $C,C^\prime, c,c^\prime>0$ be constants that depends only on $\nu, \lambda_{\sf m}, \lambda_{\sf M}$. 
%
%We proceed by a covering argument. Consider $\cN$ be a $\delta$ net of $\S^{m-1}$ in $L^2$ norm, where we set $\delta= \frac{\lambda_{\sf m}}{4\lambda_{\sf M}}$. By a volume argument (see e.g. \cite[Corollary 4.2.13]{vershynin2018high}), we have $|\cN|\leq \left(2/\delta +1\right)^n$. Moreover, by triangular inequality,
%\begin{equation}\label{eq:lower:deloc:norm}
%\begin{split}
%    \min_{\bv: \norm{\bv}_2=1}\norm{\bA \bv}_{2,\eps_n}
%    &\geq \min_{\bv\in \cN}\norm{\bA \bv}_{2,\eps_n}-\sup_{\bu:\norm{\bu}_2\leq \delta}\norm{\bA \bu}_{2,\eps_n}\\
%    &\stackrel{(a)}{\geq} \min_{\bv\in \cN}\norm{\bA \bv}_{2,\eps_n}-\norm{\bA}_{\op}\cdot \delta\\
%    &\stackrel{(b)}{\geq}\Big(\norm{\bA}_{\op}\Big)^{-1}\min_{\bv\in \cN}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq \eps_n \norm{\bA \bv}_2\Big)-\norm{\bA}_{\op}\cdot \delta\,.
%\end{split}
%\end{equation}
%In the above, $(a)$ holds by the inequality $\norm{\bu}_{2,\eps_n}\leq \norm{\bu}_2$, where $\bu=(u_i)_{i\leq p} \in \R^p$, and $(b)$ is due to the inequality 
%\begin{equation*}
%    \norm{\bu}_{2,\eps_n}\equiv \max_{\btheta:\norm{\btheta}_2\leq 1, \norm{\btheta}_{\infty}\leq \eps_n }\langle \btheta, \bu\rangle \geq \norm{\bu}_2^{-1}\sum_{i=1}^{p}u_i^2\one\big(|u_i|\leq \eps_n \norm{\bu}_2\big)\,,
%\end{equation*}
%where the inequality holds by taking $\theta_i=\norm{\bu}_2^{-1}u_i\one\big(|u_i|\leq \eps_n\norm{\bu}_2\big)$. Note that by Theorem \ref{theorem:matrix-concentration-covariance-operator}, if $m\leq C\cdot p$, where $C\equiv C_{\nu, \lambda_{\sf m},\lambda_{\sf M}}$ is small enough, then with probability at least $1-e^{-cp}$,
%\begin{equation}\label{eq:lambda:A}
%    \frac{p\lambda_{\sf m}}{2}\leq \lmin (\bA^{T}\bA)\leq \lmax (\bA^{T}\bA)\leq 2p\lambda_{\sf M}\,.
%\end{equation}
%Thus, using the bound \eqref{eq:lambda:A} in \eqref{eq:lower:deloc:norm} shows that with probability at least $1-e^{-cp}$, we have
%\begin{equation*}
%     \min_{\bv: \norm{\bv}_2=1}\norm{\bA \bv}_{2,\eps_n}\geq \sqrt{\frac{p}{2\lambda_{\sf M}}}\left(\min_{\bv\in \cN}\frac{1}{p}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq \eps_n \big(p\lambda_{\sf m}/2\big )^{1/2}\Big)-\frac{\lambda_{\sf m}}{2}\right)\,.
%\end{equation*}
%Therefore, it suffices to prove that for $C=(\lambda_{\sf m}/2)^{1/2}$ and $m\leq cp$, 
%\begin{equation}\label{eq:lower:goal}
%    \min_{\bv\in \cN}\frac{1}{p}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq C\eps_n \sqrt{p} \Big)\geq \frac{\lambda_{\sf m}}{2}~~~\text{holds with probability at least $1-e^{-c^\prime p}$}
%\end{equation}
%For the rest of the proof, we aim to prove \eqref{eq:lower:goal}. For fixed $\bv\in \cN$, note that $\big(\langle \ba_i, \bv \rangle\big)^2\one\big(\big|\langle \ba_i, \bv \rangle \big|\leq C\eps_n \sqrt{p}\big)$ is a subexponential random variable since $\ba_i$ is a subgaussian random vector. Thus, by Bernstein's inequality (cf. \cite[Theorem 2.8.2]{vershynin2018high}), we have for a fixed $\bv\in \cN$ and $t\geq 0$ that with probability at least $1-2e^{-cp(t\wedge t^2)}$,
%\begin{equation}\label{eq:bernstein}
%    \left|\frac{1}{p}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq C\eps_n \sqrt{p}\Big)-\E\bigg[\big(\langle \ba_1, \bv\rangle\big)^2\one\Big(\big|\langle \ba_1,\bv \rangle \big|\leq C\eps_n \sqrt{p}\Big)\bigg]\right|\leq t\,.
%\end{equation}
%Moreover, note that for $\bv\in \cN$,
%\begin{equation*}
%\begin{split}
%    \E\bigg[\big(\langle \ba_1, \bv\rangle\big)^2\one\Big(\big|\langle \ba_1,\bv \rangle \big|\leq C\eps_n \sqrt{p}\Big)\bigg]
%    &=\bv^{T}\bSigma \bv - \E\bigg[\big(\langle \ba_1, \bv\rangle\big)^2\one\Big(\big|\langle \ba_1,\bv \rangle \big|\geq C\eps_n \sqrt{p}\Big)\bigg]\\
%    &\stackrel{(a)}{\geq} \lambda_{\sf m}- \Big(\E\big(\langle \ba_1,\bu\rangle\big)^4\Big)^{1/2}\cdot \bigg(\P\Big(\big|\langle \ba_1,\bv \rangle \big|\geq C\eps_n\sqrt{p} \Big)\bigg)^{1/2}\\
%    &\stackrel{(b)}{\geq}\lambda_{\sf m}-Ce^{-cp\eps_n^2}\\
%    &\stackrel{(c)}{=}\lambda_{\sf m}-o_p(1)\,,
%\end{split}
%\end{equation*}
%where $(a)$ holds by Cauchy-Schwartz, $(b)$ holds since $\ba_1$ is a subgaussian vector, and $(c)$ holds since $\sqrt{p}\eps_n \to\infty$. Thus, taking $t=\lambda_{\sf m}/3$ in \eqref{eq:bernstein}, we have for large enough $p$ that
%\begin{equation*}
%    \P\bigg(\frac{1}{p}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq C\eps_n \sqrt{p}\Big)\leq \frac{\lambda_{\sf m}}{2}\bigg)\leq e^{-c p}\,.
%\end{equation*}
%Since $|\cN|\leq C^{m}$, taking a union bound over $\bv\in \cN$ in the above shows
%\begin{equation*}
%\P\bigg(\min_{\bv\in \cN}\frac{1}{p}\sum_{i=1}^{p}\big(\langle \ba_i, \bv \rangle\big)^2\one\Big(\big|\langle \ba_i, \bv \rangle \big|\leq C\eps_n \sqrt{p}\Big)\leq \frac{\lambda_{\sf m}}{2}\bigg)\leq C^m e^{-c p}\leq e^{-c^\prime p}\,,
%\end{equation*}
%where the last inequality holds for $m\leq C^\prime p$ for some $C^\prime \equiv C^\prime_{\nu, \lambda_{\sf m}, \lambda_{\sf M}}>0$. Consequently, \eqref{eq:lower:goal} holds, which concludes the proof.
%\end{proof}







%We divide our discussion into two cases based on the feature model $\bX$ we consider. 
%Below we use $c, C, \eta$ to denote constants independent of $n$. %These constants can vary from line to line. 

%One reduction to note is that $\smin(\bZ_S) = \smin(\bX_S)$ for any subset $S$ since
%$\bZ = \by \odot \bX$ where $\by \in \{\pm 1\}^n$.

%\begin{enumerate}[(A)]
%\item \label{part:min-svalue-independent-copies}
%	$\bX$ represents \emph{independent raw features} (Section XXX). Pick any subset $S$. 
%	Applying Theorem~\ref{theorem:general-result-on-min-singular-value-of-RMT}, we obtain that 
%	\begin{equation}
%	\label{eqn:one-single-prob-bound-low-singular-value}
%		\P(\smin(\bX_S) \ge c\eta \sqrt{p} - C\sqrt{|S|}) \ge 1-e^{-cn}.
%	\end{equation}
%	Above, the constants $\eta, c, C > 0$ are independent of the set size $S$. Below we fix these constants. 
%	
%	Now we wish to take a union bound over all subsets $S$ whose cardinality $|S| \le \Delta n$. 
%	A standard counting shows that the number of such sets by $e^{H(c') n}$ if $\Delta \le 1/2$ 
%	where $H(x) = -x \log x - (1-x)\log(1-x)$ is the entropy function. 
%	Now let $\Delta \le 1/2$. 
%	Then, with a union bound, we have
%	\begin{equation}
%		\P(\min_{S:|S| \le \Delta n} \smin(\bX_S) \ge (c\eta \sqrt{\gamma} - C\sqrt{\Delta}) \sqrt{n} ) \ge 1-e^{-(c-H(\Delta))n}.
%	\end{equation}
%	Now if we choose $\Delta$ to be any such that (i) $H(\Delta) \le c$ and (ii) $c\eta \sqrt{\gamma} > C\sqrt{\Delta}$. 
%	 %follows from a direct application of union bound to equation~\eqref{eqn:one-single-prob-bound-low-singular-value}.
%	 Then we attain the desired lower bound of the restricted minimum singular value of $\bX$, 
%	 completing the proof of Lemma~\ref{lemma:restricted-minimum-singular-value}. 
%\item $\bX$ represents the \emph{random features} (Section XXX) where $\bX_{l, i} = 
%	\sigma(\langle \bw_l, \bz_i \rangle)$. 




%\end{enumerate}

